Encyclopedia of emergent particles in three-dimensional crystals

The past decade has witnessed a surge of interest in exploring emergent particles in condensed matter systems. Novel particles, emerged as excitations around exotic band degeneracy points, continue to be reported in real materials and artificially engineered systems, but so far, we do not have a complete picture on all possible types of particles that can be achieved. Here, via systematic symmetry analysis and modeling, we accomplish a complete list of all possible particles in time reversal-invariant systems. This includes both spinful particles such as electron quasiparticles in solids, and spinless particles such as phonons or even excitations in electric-circuit and mechanical networks. We establish detailed correspondence between the particle, the symmetry condition, the effective model, and the topological character. This obtained encyclopedia concludes the search for novel emergent particles and provides concrete guidance to achieve them in physical systems.

==> basicinfo/merge/mergeSG1.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 1}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{t}$; $\{E|000\},\mathcal{T}$; Non-Centrosymmetric; without
SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 2}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{t}$; $\{I|000\},\mathcal{T}$; Centrosymmetric; without
SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 3}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 4}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|00\frac{1}{2}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 5}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{C_{2z}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 6}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{\sigma_{z}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 7}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{\sigma_{z}|\frac{1}{2}00\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multicolumn{1}{l}{$B$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline



\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 8}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{\sigma_{z}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 9}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{\sigma_{z}|\frac{1}{2}00\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$M$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline



\multirow{1}{*}{$U$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 10}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|000\},\{I|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG101.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 101}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline



\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 102}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{3}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}-\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}-\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 103}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,3}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,3}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 104}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,3}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{3}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}-\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}-\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 105}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 106}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,3}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{3}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}-\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}-\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 107}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 108}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$N$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 109}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}(k_{x}+k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\left[(\sigma_{1}-\sigma_{3})k_{x}+(\sigma_{1}+\sigma_{3})k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{2}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{2}(k_{x}-k_{y});$ \tabularnewline




\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $[c_{1}+c_{2}(k_{x}-k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}+k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{4}c_{3}+A_{1}c_{4}\right)k_{x}+\left(A_{6}c_{4}-A_{2}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{4}\right)k_{x}+\left(A_{2}c_{3}+A_{6}c_{4}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{4}\right)k_{x}+\left(A_{1}c_{3}+A_{4}c_{4}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{6}c_{3}+A_{2}c_{4}\right)k_{x}+\left(A_{4}c_{4}-A_{1}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 110}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$N$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}(k_{x}+k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{10},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[(k_{x}+k_{y})\Gamma_{0,1}+(k_{x}-k_{y})\Gamma_{0,3}\right]+\sum_{i=1}^{3}c_{i,1}\left[(k_{x}+k_{y})\Gamma_{i,1}-(k_{x}-k_{y})\Gamma_{i,3}+k_{z}\Gamma_{i,0}\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{2}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(k_{x}+k_{y})\sigma_{1}+c_{4}(k_{x}-k_{y})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $[c_{1}+c_{2}(k_{x}-k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}+k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{4}c_{3}+A_{1}c_{4}\right)k_{x}+\left(A_{6}c_{4}-A_{2}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{4}\right)k_{x}+\left(A_{2}c_{3}+A_{6}c_{4}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{4}\right)k_{x}+\left(A_{1}c_{3}+A_{4}c_{4}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{6}c_{3}+A_{2}c_{4}\right)k_{x}+\left(A_{4}c_{4}-A_{1}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG11.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 11}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|00\frac{1}{2}\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 12}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{C_{2z}|000\},\{I|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 13}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|000\},\{I|\frac{1}{2}00\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$B$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline



\multirow{1}{*}{$D$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 14}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|00\frac{1}{2}\},\{I|\frac{1}{2}0\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multicolumn{1}{l}{}& &\tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline

\multicolumn{1}{l}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\{R_{2},R_{4}\};$  & $h+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $h+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{2},R_{4}\};$  & $h+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $h+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
 &  & \tabularnewline
\multicolumn{3}{l}{Here, $h=(c_{1}+c_{2}k_{x}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}k_{y}+c_{5}k_{z}^{2})\sigma_{0}$.}\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 15}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{C_{2z}|000\},\{I|\frac{1}{2}00\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$A$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$M$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline



\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 16}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
















$\Lambda$;& &\tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 17}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline



\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

$D$;& &\tabularnewline
\multicolumn{1}{l}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline


\multicolumn{1}{l}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 18}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multicolumn{1}{l}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
$R$;  & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multicolumn{1}{l}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline


\multicolumn{1}{l}{$C$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline


\multicolumn{1}{l}{$H$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+c_{4}\Gamma_{1,0}k_{y}+c_{5}\Gamma_{2,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}k_{x}\Gamma_{1,i}+c_{i,2}k_{y}\Gamma_{2,i}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 19}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\{R_{5},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,3}k_{x}+c_{3}\Gamma_{0,1}k_{y}+c_{4}\Gamma_{0,2}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}-c_{4}\sigma_{2})k_{z};$ \tabularnewline
$\Sigma$;& &\tabularnewline
\multicolumn{1}{l}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multicolumn{1}{l}{$H$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{y};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{2,0}k_{x}+c_{5}\Gamma_{1,0}k_{z}+\sum_{i=1}^{3}\left(c_{i,1}k_{x}\Gamma_{1,i}+c_{i,2}k_{z}\Gamma_{2,i}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{1,0}k_{y}+c_{5}\Gamma_{2,0}k_{z}+\sum_{i=1}^{3}\left(c_{i,1}k_{z}\Gamma_{1,i}+c_{i,2}k_{y}\Gamma_{2,i}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+c_{4}\Gamma_{1,0}k_{y}+c_{5}\Gamma_{2,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}k_{x}\Gamma_{1,i}+c_{i,2}k_{y}\Gamma_{2,i}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 20}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline


\multicolumn{1}{l}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline



\multicolumn{1}{l}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

$\Delta$;& &\tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multicolumn{1}{l}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG111.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 111}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2x}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 112}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2x}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(4_{3}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(4_{3}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(4_{3}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(4_{3}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 113}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{3},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{x}k_{y};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{2,1}+c_{3}\Gamma_{2,2}\right)+c_{4}\left(\Gamma_{1,0}k_{x}+\Gamma_{1,3}k_{y}\right)+c_{5}\left(\Gamma_{2,3}k_{x}+\Gamma_{2,0}k_{y}\right)-k_{y}\left(c_{6}\Gamma_{1,1}-c_{7}\Gamma_{1,2}\right);$ \tabularnewline
 & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}-c_{3}\Gamma_{1,2}\right)+c_{4}\left(\Gamma_{1,3}k_{x}-\Gamma_{1,0}k_{y}\right)+c_{5}\left(\Gamma_{2,3}k_{y}-\Gamma_{2,0}k_{x}\right)+k_{y}\left(c_{6}\Gamma_{2,1}+c_{7}\Gamma_{2,2}\right);$ \tabularnewline
 & $\left\{ R_{3},R_{3}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{0,3}+c_{3}\Gamma_{3,3}\right)k_{x}k_{y}+\left(c_{4}\Gamma_{1,3}+c_{5}\Gamma_{2,0}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 114}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,2}k_{z}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,2}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{3},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{x}k_{y};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{2,1}+c_{3}\Gamma_{2,2}\right)+c_{4}\left(\Gamma_{1,0}k_{x}+\Gamma_{1,3}k_{y}\right)+c_{5}\left(\Gamma_{2,3}k_{x}+\Gamma_{2,0}k_{y}\right)-k_{y}\left(c_{6}\Gamma_{1,1}-c_{7}\Gamma_{1,2}\right);$ \tabularnewline
 & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}-c_{3}\Gamma_{1,2}\right)+c_{4}\left(\Gamma_{1,3}k_{x}-\Gamma_{1,0}k_{y}\right)+c_{5}\left(\Gamma_{2,3}k_{y}-\Gamma_{2,0}k_{x}\right)+k_{y}\left(c_{6}\Gamma_{2,1}+c_{7}\Gamma_{2,2}\right);$ \tabularnewline
 & $\left\{ R_{3},R_{3}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{0,3}+c_{3}\Gamma_{3,3}\right)k_{x}k_{y}+\left(c_{4}\Gamma_{1,3}+c_{5}\Gamma_{2,0}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 115}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2a}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 116}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2a}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline



\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 117}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2a}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 118}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2a}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 119}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\{C_{2a}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 120}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\{C_{2a}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$N$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{3}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG121.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 121}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}k_{z}+c_{5}k_{x}k_{y})\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 122}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\{C_{2x}|\frac{1}{4}\frac{3}{4}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}(k_{x}+k_{y});$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{y}+\sigma_{2}k_{x});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{y}+\sigma_{2}k_{x});$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{2}(k_{x}-k_{y});$ \tabularnewline




\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}-k_{y})\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}+k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 123}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 124}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{3}\sigma_{2}(k_{x}-k_{y})+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 125}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{2}(k_{x}^{2}-k_{y}^{2})+c_{6}\sigma_{3}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 126}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{2}(k_{x}^{2}-k_{y}^{2})+c_{6}\sigma_{3}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{2}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 127}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left(c_{2}\Gamma_{1,0}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}+c_{3}\Gamma_{2,3}\right)\left(k_{x}-k_{y}\right)-\left(c_{3}\Gamma_{1,0}-c_{3}\Gamma_{1,3}+c_{2}\Gamma_{2,0}-c_{2}\Gamma_{2,3}\right)\left(k_{x}+k_{y}\right)+\left[(1+i)\left(c_{3}+ic_{2}\right)\left(\Gamma_{2,+}k_{+}+\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
 & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{7},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right)k_{x}k_{y};$\tabularnewline
 & $\left\{ R_{7},R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left[c_{2}\left(\Gamma_{1,0}+\Gamma_{1,3}\right)-c_{3}\left(\Gamma_{2,0}+\Gamma_{2,3}\right)\right]\left(k_{x}+k_{y}\right)+\left[c_{2}\left(\Gamma_{2,0}-\Gamma_{2,3}\right)-c_{3}\left(\Gamma_{1,0}-\Gamma_{1,3}\right)\right]\left(k_{x}-k_{y}\right)+\left[(1+i)\left(c_{2}+ic_{3}\right)\left(\Gamma_{2,+}k_{+}-\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{0,1}+c_{3}\Gamma_{0,2}+c_{4}\Gamma_{3,1}+c_{5}\Gamma_{3,2}\right)+k_{z}\left(c_{6}\Gamma_{1,0}+c_{7}\Gamma_{2,3}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{0,1}+c_{3}\Gamma_{0,2}+c_{4}\Gamma_{3,1}+c_{5}\Gamma_{3,2}\right)+k_{z}\left(c_{6}\Gamma_{1,0}+c_{7}\Gamma_{2,3}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 128}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,2}k_{z}+\sum_{i=1}^{2}\left[c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{2}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left(c_{2}\Gamma_{1,0}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}+c_{3}\Gamma_{2,3}\right)\left(k_{x}-k_{y}\right)-\left(c_{3}\Gamma_{1,0}-c_{3}\Gamma_{1,3}+c_{2}\Gamma_{2,0}-c_{2}\Gamma_{2,3}\right)\left(k_{x}+k_{y}\right)+\left[(1+i)\left(c_{3}+ic_{2}\right)\left(\Gamma_{2,+}k_{+}+\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
 & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{7},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right)k_{x}k_{y};$\tabularnewline
 & $\left\{ R_{7},R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left[c_{2}\left(\Gamma_{1,0}+\Gamma_{1,3}\right)-c_{3}\left(\Gamma_{2,0}+\Gamma_{2,3}\right)\right]\left(k_{x}+k_{y}\right)+\left[c_{2}\left(\Gamma_{2,0}-\Gamma_{2,3}\right)-c_{3}\left(\Gamma_{1,0}-\Gamma_{1,3}\right)\right]\left(k_{x}-k_{y}\right)+\left[(1+i)\left(c_{2}+ic_{3}\right)\left(\Gamma_{2,+}k_{+}-\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{0,1}+c_{3}\Gamma_{0,2}+c_{4}\Gamma_{3,1}+c_{5}\Gamma_{3,2}\right)+k_{z}\left(c_{6}\Gamma_{1,0}+c_{7}\Gamma_{2,3}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 129}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}+\Gamma_{1,2}+\Gamma_{2,1}-\Gamma_{2,2}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}-\Gamma_{1,2}+\Gamma_{2,1}+\Gamma_{2,2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right]$\tabularnewline
 & $\left\{ R_{2},R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,1}-\Gamma_{1,2}-\Gamma_{2,1}+\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,1}+\Gamma_{1,2}-\Gamma_{2,1}-\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 130}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{9},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,1}k_{z}+c_{5}\Gamma_{0,3}(k_{x}^{2}-k_{y}^{2})+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{13},R_{14}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,3}(k_{x}^{2}-k_{y}^{2})+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,3}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{3,1}k_{x}+c_{3}\Gamma_{0,2}k_{z}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{2}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}+\Gamma_{1,2}+\Gamma_{2,1}-\Gamma_{2,2}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}-\Gamma_{1,2}+\Gamma_{2,1}+\Gamma_{2,2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right]$\tabularnewline
 & $\left\{ R_{2},R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,1}-\Gamma_{1,2}-\Gamma_{2,1}+\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,1}+\Gamma_{1,2}-\Gamma_{2,1}-\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG131.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 131}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 132}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|000\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline



\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 133}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,3}k_{x}k_{y}+c_{4}\Gamma_{i,0}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{2}(k_{x}^{2}-k_{y}^{2})+c_{6}\sigma_{3}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 134}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{2}(k_{x}^{2}-k_{y}^{2})+c_{6}\sigma_{3}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 135}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{9},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,1}k_{z}+c_{5}\Gamma_{0,3}(k_{x}^{2}-k_{y}^{2})+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{13},R_{14}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,3}(k_{x}^{2}-k_{y}^{2})+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,3}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left(c_{2}\Gamma_{1,0}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}+c_{3}\Gamma_{2,3}\right)\left(k_{x}-k_{y}\right)-\left(c_{3}\Gamma_{1,0}-c_{3}\Gamma_{1,3}+c_{2}\Gamma_{2,0}-c_{2}\Gamma_{2,3}\right)\left(k_{x}+k_{y}\right)+\left[(1+i)\left(c_{3}+ic_{2}\right)\left(\Gamma_{2,+}k_{+}+\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
 & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{7},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right)k_{x}k_{y};$\tabularnewline
 & $\left\{ R_{7},R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left[c_{2}\left(\Gamma_{1,0}+\Gamma_{1,3}\right)-c_{3}\left(\Gamma_{2,0}+\Gamma_{2,3}\right)\right]\left(k_{x}+k_{y}\right)+\left[c_{2}\left(\Gamma_{2,0}-\Gamma_{2,3}\right)-c_{3}\left(\Gamma_{1,0}-\Gamma_{1,3}\right)\right]\left(k_{x}-k_{y}\right)+\left[(1+i)\left(c_{2}+ic_{3}\right)\left(\Gamma_{2,+}k_{+}-\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 136}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left(c_{2}\Gamma_{1,0}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}+c_{3}\Gamma_{2,3}\right)\left(k_{x}-k_{y}\right)-\left(c_{3}\Gamma_{1,0}-c_{3}\Gamma_{1,3}+c_{2}\Gamma_{2,0}-c_{2}\Gamma_{2,3}\right)\left(k_{x}+k_{y}\right)+\left[(1+i)\left(c_{3}+ic_{2}\right)\left(\Gamma_{2,+}k_{+}+\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
 & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{7},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right)k_{x}k_{y};$\tabularnewline
 & $\left\{ R_{7},R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left[c_{2}\left(\Gamma_{1,0}+\Gamma_{1,3}\right)-c_{3}\left(\Gamma_{2,0}+\Gamma_{2,3}\right)\right]\left(k_{x}+k_{y}\right)+\left[c_{2}\left(\Gamma_{2,0}-\Gamma_{2,3}\right)-c_{3}\left(\Gamma_{1,0}-\Gamma_{1,3}\right)\right]\left(k_{x}-k_{y}\right)+\left[(1+i)\left(c_{2}+ic_{3}\right)\left(\Gamma_{2,+}k_{+}-\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 137}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,2}k_{z}+\sum_{i=1}^{2}\left[c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}+\Gamma_{1,2}+\Gamma_{2,1}-\Gamma_{2,2}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}-\Gamma_{1,2}+\Gamma_{2,1}+\Gamma_{2,2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right]$\tabularnewline
 & $\left\{ R_{2},R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,1}-\Gamma_{1,2}-\Gamma_{2,1}+\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,1}+\Gamma_{1,2}-\Gamma_{2,1}-\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 138}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{3,1}k_{x}+c_{3}\Gamma_{0,2}k_{z}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}+\Gamma_{1,2}+\Gamma_{2,1}-\Gamma_{2,2}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}-\Gamma_{1,2}+\Gamma_{2,1}+\Gamma_{2,2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right]$\tabularnewline
 & $\left\{ R_{2},R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,1}-\Gamma_{1,2}-\Gamma_{2,1}+\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,1}+\Gamma_{1,2}-\Gamma_{2,1}-\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 139}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}k_{x}k_{y}+c_{5}k_{z})\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sigma_{1}\left(c_{5}k_{x}+c_{6}k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 140}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG141.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 141}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|0\frac{1}{2}0\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}(k_{x}+k_{y});$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}(k_{x}+k_{y});$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{2}k_{x}+\sigma_{1}k_{y});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{2}k_{x}+\sigma_{1}k_{y});$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}(k_{x}-k_{y})+c_{4}\sigma_{3}(k_{x}+k_{y});$ \tabularnewline




\multirow{1}{*}{$U$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{3}\sigma_{3}(k_{x}-k_{y})+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}-k_{y})\right]\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{9}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sigma_{1}\left(c_{5}k_{x}+c_{6}k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 142}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{1}{2}00\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}(c_{2}k_{z}+c_{3}k_{x});$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & \multirow{1}{*}{$\{R_{13},R_{14}\};$ } & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,2}k_{x}+\Gamma_{0,1}k_{y}\right)+c_{3}\left(\Gamma_{2,0}k_{x}-\Gamma_{1,3}k_{y}\right)$ \tabularnewline
 &  & $+c_{4}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,3}k_{y}\right)+k_{z}\left(c_{4}\Gamma_{1,1}-c_{6}\Gamma_{2,1}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{10};$  & $h_{0}^{\prime}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{3}(k_{x}-k_{y});$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{3}\sigma_{3}(k_{x}-k_{y})+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}-k_{y})\right]\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{9}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 143}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 144}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{1}{3}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 145}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{2}{3}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 146}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{C_{3}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 147}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{+}+\alpha_{2}k_{-}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{+}+\alpha_{2}k_{-}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 148}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{S_{6}^{+}|000\},\mathcal{T}$; Centrosymmetric;
without SOC}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{+}+\alpha_{2}k_{-}^{2})+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{+}+\alpha_{2}k_{-}^{2})+h.c.\right];$ \tabularnewline



\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 149}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 150}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}-\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG151.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 151}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{1}{3}\},\{C_{21}^{\prime}|00\frac{2}{3}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}[b]{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 152}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{1}{3}\},\{C_{21}^{\prime\prime}|00\frac{2}{3}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}[b]{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}-\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$T'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$S'$;} & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 153}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{2}{3}\},\{C_{21}^{\prime}|00\frac{1}{3}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 154}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{2}{3}\},\{C_{21}^{\prime\prime}|00\frac{1}{3}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}-\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$T'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$S'$;} & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 155}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(k_{x}+\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+c_{3}k_{z}\right]+\sigma_{2}\left[c_{4}\left(\frac{k_{y}}{\sqrt{3}}-k_{x}\right)-c_{5}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sum_{i=0,3}\sigma_{i}c_{i,2}\left(k_{x}-\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{3}k_{z}\right]+\sigma_{2}\left[c_{4}\left(3k_{x}+\sqrt{3}k_{y}\right)+3c_{5}k_{z}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 156}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{\sigma_{v1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right];$ \tabularnewline



\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{3}k_{x}-\sigma_{1}k_{y});$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left[2A_{4}c_{3}+\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}-2A_{1}c_{6}\right]k_{x}+2\left(A_{6}c_{3}-A_{7}c_{4}-A_{2}c_{6}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left[2A_{6}c_{3}+\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}-2A_{2}c_{6}\right]k_{x}-2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 157}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{\sigma_{d1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multirow{1}{*}{$S'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 158}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{\sigma_{v1}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,3}k_{x}+\Gamma_{0,1}k_{y}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+\sigma_{3}(c_{2}k_{x}+c_{3}k_{z});$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}k_{z}\sigma_{i};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}k_{z}\sigma_{i};$ \tabularnewline
 & $\{R_{3},R_{3}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}k_{z}\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{3}k_{x}-\sigma_{1}k_{y});$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+\sqrt{3}c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}(k_{x}-\sqrt{3}k_{y})+c_{i,2}k_{z}\right]\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left[2A_{4}c_{3}+\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}-2A_{1}c_{6}\right]k_{x}+2\left(A_{6}c_{3}-A_{7}c_{4}-A_{2}c_{6}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left[2A_{6}c_{3}+\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}-2A_{2}c_{6}\right]k_{x}-2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 159}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{\sigma_{d1}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}-\Gamma_{0,3}k_{y}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+\sigma_{3}(c_{2}k_{y}+c_{3}k_{z});$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{6};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}-\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline





\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multirow{1}{*}{$S'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 160}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{C_{3}^{+}|000\},\{\sigma_{d1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline



\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG161.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 161}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{C_{3}^{+}|000\},\{\sigma_{d1}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}-\Gamma_{0,3}k_{y}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+\left[c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{3}k_{z}\right]\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+\sqrt{3}c_{2}k_{x}-c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}(\sqrt{3}k_{x}+k_{y})+c_{i,2}k_{z}\right]\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 162}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+c_{2}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+c_{2}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 163}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime}|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,2}k_{x}+\Gamma_{3,1}k_{y}\right)+k_{z}\left(c_{4}\Gamma_{1,2}+c_{3}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{6};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline





\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{3}k_{x})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+c_{2}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+c_{2}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 164}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime\prime}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}-c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}-c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\left(\sigma_{3}k_{x}-\sigma_{1}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+\sigma_{1}\left(c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{2}\left(c_{2}k_{y}-c_{3}k_{x}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(\left(c_{3}+c_{4}\right)k_{z}+c_{1}\right)+\sigma_{3}\left(\left(c_{3}-c_{4}\right)k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z}-2\left(A_{7}c_{3}+A_{2}c_{5}\right)k_{y}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{3}-2A_{1}c_{5}\right]k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{4}+c_{5}k_{z}\right)-2\left(A_{7}c_{3}-A_{1}c_{6}\right)k_{y}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{3}-2A_{2}c_{6}\right]k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sum_{i=0,3}\sigma_{i}\left[c_{i,1}+c_{i,2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{1}\left[c_{1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sum_{i=0,3}\sigma_{i}\left[c_{i,1}+c_{i,2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{1}\left[c_{1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{y}+\sigma_{1}\left(c_{2}k_{x}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{y}+\sigma_{1}\left(c_{2}k_{x}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 165}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime\prime}|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}-c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,1}k_{x}-\Gamma_{0,2}k_{y}\right)+k_{z}\left(c_{4}\Gamma_{1,2}+c_{3}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\left(\Gamma_{i,1}k_{x}-\Gamma_{i,3}k_{y}\right)+c_{i,2}k_{z}\Gamma_{i,2}\right];$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{3}k_{x}-\sigma_{1}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+\sigma_{1}\left(c_{3}k_{x}+c_{4}k_{y}\right)-\sigma_{2}\left(c_{4}k_{x}-c_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sqrt{3}c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}(k_{x}-\sqrt{3}k_{y})+c_{i,2}k_{z}\right]\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline


\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(\left(c_{3}+c_{4}\right)k_{z}+c_{1}\right)+\sigma_{3}\left(\left(c_{3}-c_{4}\right)k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z}-2\left(A_{7}c_{3}+A_{2}c_{5}\right)k_{y}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{3}-2A_{1}c_{5}\right]k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{4}+c_{5}k_{z}\right)-2\left(A_{7}c_{3}-A_{1}c_{6}\right)k_{y}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{3}-2A_{2}c_{6}\right]k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sum_{i=0,3}\sigma_{i}\left[c_{i,1}+c_{i,2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{1}\left[c_{1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{y}+\sigma_{1}\left(c_{2}k_{x}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 166}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline



\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(k_{x}+\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(\sqrt{3}k_{x}-k_{y}\right)+c_{3}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{3}k_{z}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 167}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,2}k_{x}+\Gamma_{3,1}k_{y}\right)+k_{z}\left(c_{4}\Gamma_{1,2}+c_{3}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left[c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{3}k_{z}\right];$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x}-c_{2}\sqrt{3}k_{y})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}(\sqrt{3}k_{x}+k_{y})+c_{i,2}k_{z}\right]\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(k_{x}+\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(\sqrt{3}k_{x}-k_{y}\right)+c_{3}k_{z}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 168}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 169}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{6}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{2},R_{12}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 170}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{5}{6}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{2},R_{12}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG171.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 171}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{3}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 172}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{2}{3}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 173}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{2}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{2},R_{12}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 174}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline



\multirow{1}{*}{$\Delta$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\sqrt{3}A_{1}\left(c_{3}-2c_{4}\right)+\sqrt{3}A_{2}\left(c_{4}-2c_{3}\right)+3\left(A_{4}c_{3}+A_{6}c_{4}\right)\right]k_{x}+3\left(A_{1}c_{3}-A_{2}c_{4}\right)k_{y}+\sqrt{3}\left[\left(2A_{4}+A_{6}\right)c_{4}-\left(A_{4}+2A_{6}\right)c_{3}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 175}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{2}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{11},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{11},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{6}\};$  & $c_{3}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{2}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{6}\};$  & $c_{3}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{2}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+\sigma_{1}\left(c_{3}k_{x}+c_{4}k_{y}\right)-\sigma_{2}\left(c_{4}k_{x}-c_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{5}+c_{6}k_{z}\right)+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{6}k_{z}+c_{10}k^{2}+c_{11}k_{z}^{2}\right)+2\left[2\left(A_{1}-A_{2}\right)c_{5}+2A_{3}c_{7}+\left(A_{4}+A_{6}\right)c_{8}+A_{7}c_{9}\right]k_{x}k_{y}+\left[2\left(A_{4}+A_{6}\right)c_{5}+2A_{7}c_{7}+\left(A_{2}-A_{1}\right)c_{8}-A_{3}c_{9}\right]\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+A_{8}\left(c_{7}k_{z}+c_{10}k^{2}+c_{11}k_{z}^{2}\right)+2\left[-2A_{1}c_{5}+2\left(A_{2}-A_{3}\right)c_{6}+A_{4}c_{8}+\left(A_{6}+A_{7}\right)c_{9}\right]k_{x}k_{y}+\left[2A_{4}c_{5}+2\left(A_{6}+A_{7}\right)c_{6}+A_{1}c_{8}+\left(A_{3}-A_{2}\right)c_{9}\right]\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{3},R_{5}\right\} ;$  & $\Gamma_{1,0}\left(c_{3}k_{x}+c_{4}k_{y}\right)+\Gamma_{2,3}\left(c_{3}k_{y}-c_{4}k_{x}\right)+\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+\Gamma_{3,0}\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3},R_{5}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}\left(c_{5}+c_{6}k_{z}\right)+\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{5}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 176}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{2}|00\frac{1}{2}\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{11},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{13},R_{15}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,3}k_{z}+\left(\alpha_{1}\Gamma_{+,1}k_{-}^{2}+\alpha_{2}k_{z}\Gamma_{+,0}k_{+}+h.c.\right)$; \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $\{R_{2},R_{6}\};$  & $c_{3}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{2}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}k_{z}+h.c.\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}k_{z}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+\sigma_{1}\left(c_{3}k_{x}+c_{4}k_{y}\right)-\sigma_{2}\left(c_{4}k_{x}-c_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{5}+c_{6}k_{z}\right)+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{6}k_{z}+c_{10}k^{2}+c_{11}k_{z}^{2}\right)+2\left[2\left(A_{1}-A_{2}\right)c_{5}+2A_{3}c_{7}+\left(A_{4}+A_{6}\right)c_{8}+A_{7}c_{9}\right]k_{x}k_{y}+\left[2\left(A_{4}+A_{6}\right)c_{5}+2A_{7}c_{7}+\left(A_{2}-A_{1}\right)c_{8}-A_{3}c_{9}\right]\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+A_{8}\left(c_{7}k_{z}+c_{10}k^{2}+c_{11}k_{z}^{2}\right)+2\left[-2A_{1}c_{5}+2\left(A_{2}-A_{3}\right)c_{6}+A_{4}c_{8}+\left(A_{6}+A_{7}\right)c_{9}\right]k_{x}k_{y}+\left[2A_{4}c_{5}+2\left(A_{6}+A_{7}\right)c_{6}+A_{1}c_{8}+\left(A_{3}-A_{2}\right)c_{9}\right]\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{3},R_{5}\right\} ;$  & $\Gamma_{1,0}\left(c_{3}k_{x}+c_{4}k_{y}\right)+\Gamma_{2,3}\left(c_{3}k_{y}-c_{4}k_{x}\right)+\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+\Gamma_{3,0}\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3},R_{5}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}\left(c_{5}+c_{6}k_{z}\right)+\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{5}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 177}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 178}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{6}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{2},R_{8}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{2},R_{4}\};$  & $\sigma_{0}\left(c_{2}k_{y}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 179}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{5}{6}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{2},R_{8}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{2},R_{4}\};$  & $\sigma_{0}\left(c_{2}k_{y}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 180}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{3}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG181.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 181}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{2}{3}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 182}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{2}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{2},R_{8}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$S'$;} & $\{R_{2},R_{4}\};$  & $\sigma_{0}\left(c_{2}k_{y}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 183}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|000\},\{\sigma_{v1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{6}\left(A_{4}k_{x}+A_{6}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{6}c_{5}-A_{2}c_{6}\right)k_{x}+\left(A_{1}c_{6}-A_{4}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{4}c_{5}-A_{1}c_{6}\right)k_{x}+\left(A_{2}c_{6}-A_{6}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{6}\left(A_{6}k_{x}+A_{4}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,2}k_{y}-\Gamma_{2,0}k_{x}\right)+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 184}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|000\},\{\sigma_{v1}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,3}\left(k_{x}^{2}-k_{y}^{2}\right)-2c_{i,2}\Gamma_{i,1}k_{x}k_{y}\right];$ \tabularnewline
 & $\{R_{9},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{12},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,3}\left(k_{x}^{2}-k_{y}^{2}\right)-2c_{i,2}\Gamma_{i,1}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\left(\Gamma_{i,1}k_{x}-\Gamma_{i,3}k_{y}\right)\right];$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right)+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$S'$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+\left(c_{2}\sigma_{1}+c_{4}\sigma_{2}\right)k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{2}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{6}\left(A_{4}k_{x}+A_{6}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{6}c_{5}-A_{2}c_{6}\right)k_{x}+\left(A_{1}c_{6}-A_{4}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{4}c_{5}-A_{1}c_{6}\right)k_{x}+\left(A_{2}c_{6}-A_{6}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{6}\left(A_{6}k_{x}+A_{4}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,2}k_{y}-\Gamma_{2,0}k_{x}\right)+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 185}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{2}\},\{\sigma_{v1}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{5},R_{11}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,0}k_{z}+c_{5}\left[2\Gamma_{0,1}k_{x}k_{y}+\Gamma_{0,3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+\left[\alpha_{1}k_{z}\left(k_{x}\Gamma_{+,1}+k_{y}\Gamma_{+,3}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $c_{1}\sigma_{0}+\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z};$ \tabularnewline
 & $\{R_{3},R_{3}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}+\Gamma_{0,3}k_{y}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{6}\left(A_{4}k_{x}+A_{6}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{6}c_{5}-A_{2}c_{6}\right)k_{x}+\left(A_{1}c_{6}-A_{4}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{4}c_{5}-A_{1}c_{6}\right)k_{x}+\left(A_{2}c_{6}-A_{6}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{6}\left(A_{6}k_{x}+A_{4}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,2}k_{y}-\Gamma_{2,0}k_{x}\right)+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+\left[\left(\alpha_{1}\Gamma_{1,+}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}\right)\left(k_{x}-\sqrt{3}k_{y}\right)+\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}+c_{4}\Gamma_{0,3}+c_{5}\Gamma_{3,3}\right)k_{z}+h.c.\right];$\tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{y}+\left[\left(\alpha_{1}\Gamma_{2,+}+c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)k_{x}+\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}+c_{4}\Gamma_{0,3}+c_{5}\Gamma_{3,3}\right)k_{z}+h.c.\right];$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 186}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{2}\},\{\sigma_{v1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{5},R_{11}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,0}k_{z}+c_{5}\left[2\Gamma_{0,1}k_{x}k_{y}+\Gamma_{0,3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+\left[\alpha_{1}k_{z}\left(k_{x}\Gamma_{+,3}-k_{y}\Gamma_{+,1}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}k_{z}-\sigma_{3}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{6}\left(A_{4}k_{x}+A_{6}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{6}c_{5}-A_{2}c_{6}\right)k_{x}+\left(A_{1}c_{6}-A_{4}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{4}c_{5}-A_{1}c_{6}\right)k_{x}+\left(A_{2}c_{6}-A_{6}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{6}\left(A_{6}k_{x}+A_{4}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,2}k_{y}-\Gamma_{2,0}k_{x}\right)+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}+c_{i,2}k_{x}\right)+\left[k_{y}\left(\alpha_{1}\Gamma_{1,+}+c_{1}\Gamma_{1,3}+c_{2}\Gamma_{2,0}\right)+k_{z}\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}+c_{3}\Gamma_{0,3}+c_{4}\Gamma_{3,3}\right)+h.c.\right];$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 187}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline



\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{3}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(\frac{k_{x}}{\sqrt{3}}+k_{y}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sqrt{3}\sigma_{2}-3\sigma_{1}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(\frac{k_{x}}{\sqrt{3}}+k_{y}\right)\right];$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 188}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\{C_{21}^{\prime}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\left(\Gamma_{0,1}k_{x}-\Gamma_{3,2}k_{y}\right)k_{z}+\left[2\alpha_{1}k_{x}k_{y}\Gamma_{+,0}+i\alpha_{1}\Gamma_{+,3}\left(k_{x}^{2}-k_{y}^{2}\right)+\alpha_{2}k_{z}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{5}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{3},R_{6}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{3}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(\frac{k_{x}}{\sqrt{3}}+k_{y}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sqrt{3}\sigma_{2}-3\sigma_{1}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(\frac{k_{x}}{\sqrt{3}}+k_{y}\right)\right];$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 189}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\{C_{21}^{\prime\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 190}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\{C_{21}^{\prime\prime}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\left(\Gamma_{0,1}k_{y}+\Gamma_{3,2}k_{x}\right)k_{z}+\left[2\alpha_{1}k_{x}k_{y}\Gamma_{+,0}+i\alpha_{1}\Gamma_{+,3}\left(k_{x}^{2}-k_{y}^{2}\right)+\alpha_{2}k_{z}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{7};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)k_{z};$ \tabularnewline
 & $R_{8};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left(\sigma_{2}k_{x}-\sigma_{1}k_{y}\right)k_{z};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{3}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$S'$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG191.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 191}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\{C_{2}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+k_{z}\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 192}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|00\frac{1}{2}\},\{C_{2}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\left[2\alpha_{1}k_{x}k_{y}\Gamma_{+,0}+i\alpha_{1}\Gamma_{+,3}\left(k_{x}^{2}-k_{y}^{2}\right)+\alpha_{2}k_{z}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
 & $\{R_{16},R_{17}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\left[2\alpha_{1}k_{x}k_{y}\Gamma_{+,0}+i\alpha_{1}\Gamma_{+,3}\left(k_{x}^{2}-k_{y}^{2}\right)+\alpha_{2}k_{z}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
 & $R_{18};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+\left[\alpha_{1}\left(k_{x}\Gamma_{+,3}+ik_{y}\Gamma_{+,0}\right)+\alpha_{2}k_{z}\Gamma_{+,1}+h.c.\right];$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{3}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+k_{z}\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 193}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\{C_{2}|00\frac{1}{2}\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{15};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,3}k_{z}+c_{5}k_{z}\left(\Gamma_{3,2}k_{x}+\Gamma_{0,1}k_{y}\right)+\left[c_{4}\Gamma_{+,0}\left(k_{x}^{2}-k_{y}^{2}\right)-2ic_{4}k_{x}k_{y}\Gamma_{+,3}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}+\Gamma_{0,3}k_{y}\right)+k_{z}\left(c_{3}\Gamma_{1,0}+c_{4}\Gamma_{2,0}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+k_{z}\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+\left[\alpha_{1}\Gamma_{1,+}\left(k_{x}-\sqrt{3}k_{y}\right)+\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}\right)k_{z}+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}+c_{i,2}k_{y}\right)+\left[\alpha_{1}k_{x}\Gamma_{1,+}+k_{z}\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 194}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|00\frac{1}{2}\},\{C_{2}|00\frac{1}{2}\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{15};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,3}k_{z}+c_{5}k_{z}\left(\Gamma_{0,1}k_{x}-\Gamma_{3,2}k_{y}\right)+\left[c_{6}\Gamma_{+,0}\left(k_{x}^{2}-k_{y}^{2}\right)-2ic_{6}k_{x}k_{y}\Gamma_{+,3}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{7};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(ic_{4}k_{+}k_{z}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $R_{8};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(ic_{4}k_{-}k_{z}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+k_{z}\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{z}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 195}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline


\multirow{1}{*}{$R$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x}+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 196}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline

\multirow{1}{*}{$L$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(q_{x}^{2}+q_{y}^{2})+c_{3}q_{z}^{2}\right]\sigma_{0}+c_{4}q_{z}\sigma_{3}+\left[\sigma_{+}\left(\alpha_{1}q_{+}^{2}+\alpha_{2}q_{z}q_{-}\right)+h.c\right];$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 197}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right)+c_{3}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{-}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 198}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{+}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i,1}k_{i}^{2}\right)\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{x}k_{y}+h.c.\right];$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i,1}k_{i}^{2}\right)\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{x}k_{y}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{4},R_{4}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}-\Gamma_{0,2}k_{y}-\Gamma_{0,3}k_{z}\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,1}k_{x}-\Gamma_{0,2}k_{y}-\Gamma_{3,3}k_{z}\right);$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{3}k_{z}+c_{1}\right)+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{2}\};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i,1}k_{i}^{2}\right)+c_{3}\sigma_{3}k_{x}k_{y}+\left[\alpha_{1}\sigma_{+}k_{x}k_{y}+h.c.\right];$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i,1}k_{i}^{2}\right)+c_{3}\sigma_{3}k_{x}k_{y}+\left[\alpha_{1}\sigma_{+}k_{x}k_{y}+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\Gamma_{2,0}k_{x}+c_{3}\Gamma_{1,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,2}\Gamma_{1,i}k_{x}+c_{i,3}\Gamma_{2,i}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 199}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{+}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]\sigma_{1}+\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]\sigma_{2}+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{5},R_{6}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\left[c_{3}(k_{x}^{2}-k_{y}^{2})+c_{4}(k_{z}^{2}-k_{y}^{2})\right]\sigma_{1}+\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]\sigma_{2}+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{8};$  & $A_{0}c_{1}+c_{2}\left(A_{3}k_{x}+A_{1}k_{y}-A_{2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}q_{z}\sigma_{3}+c_{2}\left(q_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}q_{z}\sigma_{3}+c_{2}\left(q_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}q_{z}\sigma_{3}+c_{2}\left(q_{-}\sigma_{+}+h.c.\right);$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{-}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 200}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline


\multirow{1}{*}{$R$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left(c_{4}q_{x}-c_{5}q_{y}\right)\left(A_{4}+A_{6}\right)+\left(c_{4}q_{y}+c_{5}q_{x}\right)\left(A_{1}-A_{2}\right)+A_{7}\left(c_{6}q_{x}-c_{7}q_{y}\right)+A_{3}\left(c_{7}q_{x}+c_{6}q_{y}\right);$\tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{z}\right)+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG201.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 201}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline

\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{z}\right)+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 202}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline

\multirow{1}{*}{$L$;}&  $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2})\sigma_{0}+\left[(\alpha_{1}q_{+}^{2}+\alpha_{2}q_{z}q_{-})\sigma_{+}+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2})\sigma_{0}+\left[(\alpha_{1}q_{-}^{2}+\alpha_{2}q_{z}q_{+})\sigma_{+}+h.c.\right];$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{z}\right)+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 203}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{+}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$L$;}&  $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2})\sigma_{0}+\left[(\alpha_{1}q_{+}^{2}+\alpha_{2}q_{z}q_{-})\sigma_{+}+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2})\sigma_{0}+\left[(\alpha_{1}q_{-}^{2}+\alpha_{2}q_{z}q_{+})\sigma_{+}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{9};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{z}\right)+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 204}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{S_{61}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}(q_{+}^{2}+2\sqrt{2}q_{-}q_{z})\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z});$ \tabularnewline



\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline


\multirow{1}{*}{$F$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}p_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}p_{-}+h.c.);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}-\left[c_{4}\left(A_{4}+A_{6}\right)+A_{7}c_{5}\right]\left(\sqrt{3}p_{x}+p_{y}\right)+\left[c_{4}\left(A_{1}-A_{2}\right)+A_{3}c_{5}\right]\left(p_{x}-\sqrt{3}p_{y}\right)+c_{6}\left[\left(A_{2}-A_{1}\right)p_{x}+\left(A_{4}+A_{6}\right)p_{y}\right]+c_{7}\left(A_{7}p_{y}-A_{3}p_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 205}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{+}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+k_{y}\left(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{4},R_{4}\};$  & $(c_{1}+c_{2}q^{2})\Gamma_{0,0}+\sum_{i}c_{1,i}\left\{ \Gamma_{i,3}\left(q_{x}^{2}+q_{y}^{2}-2q_{z}^{2}\right)-\left[\sqrt{2}e^{i\frac{7\pi}{12}}\Gamma_{i,+}\left(\sqrt{2}q_{+}q_{z}-q_{-}^{2}\right)+h.c.\right]\right\} ;$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $c_{1}\Gamma_{0,0};$ \tabularnewline
 & $\{R_{11},R_{11}\};$  & $(c_{1}+c_{2}q^{2})\Gamma_{0,0}+\sum_{i}c_{1,i}\left\{ \Gamma_{i,3}\left(q_{x}^{2}+q_{y}^{2}-2q_{z}^{2}\right)-\left[\sqrt{2}e^{i\frac{7\pi}{12}}\Gamma_{i,+}\left(\sqrt{2}q_{+}q_{z}-q_{-}^{2}\right)+h.c.\right]\right\} ;$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $c_{1}\Gamma_{0,0};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{5}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\Gamma_{0,0}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{i,3}k_{x}+c_{i,2}\Gamma_{i,1}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}c_{5}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{0,1}-c_{3}\Gamma_{0,2}+c_{4}\Gamma_{3,1}+c_{5}\Gamma_{3,2}\right)+k_{z}\left(c_{6}\Gamma_{1,1}-c_{7}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 206}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{S_{61}^{+}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{5},R_{6}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{+}q_{z}+q_{-}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $A_{0}c_{1}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{y}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{x}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{z}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{6}k_{x}k_{y}+A_{4}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{13},R_{14}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{+}q_{z}+q_{-}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{16};$  & $A_{0}c_{1}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{y}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{x}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{z}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{6}k_{x}k_{y}+A_{4}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{7},R_{7}\};$  & $c_{1}\Gamma_{0,0}+\sum_{i=1}^{3}c_{i,1}\left[\Gamma_{i,3}q_{z}+\left((-1)^{5/12}q_{-}\Gamma_{i,+}+h.c.\right)\right]$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline
\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+\sigma_{1}\left(c_{3}k_{x}+c_{4}k_{y}\right)+\sigma_{2}\left(c_{5}k_{x}+c_{6}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$F$;} & $\{R_{2},R_{6}\};$  & $\left(c_{1}+c_{2}p_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}p_{+}+h.c.);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{$ $}\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}c_{5}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+A_{8}c_{3}p_{z}+\left[\left(\sqrt{3}A_{4}+A_{1}\right)c_{5}+\left[\sqrt{3}\left(A_{6}+A_{7}\right)+A_{3}-A_{2}\right]c_{4}-A_{1}c_{6}+\left(A_{3}-A_{2}\right)c_{7}\right]p_{x}+\left[\left(A_{4}-\sqrt{3}A_{1}\right)c_{5}+\left[\sqrt{3}\left(A_{2}-A_{3}\right)+A_{6}+A_{7}\right]c_{4}+A_{4}c_{6}+\left(A_{6}+A_{7}\right)c_{7}\right]p_{y}$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 207}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,1}k_{y}\right)+c_{2}\sigma_{2}\left(k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+c_{2}\sigma_{2}\left(k_{z}-k_{x}\right)+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+c_{2}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left\{ \sigma_{+}\left[c_{2}\left(k_{x}^{2}-k_{y}^{2}\right)+ic_{3}k_{x}k_{y}\right]+h.c.\right\} ;$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left\{ \sigma_{+}\left[c_{2}\left(k_{x}^{2}-k_{y}^{2}\right)+ic_{3}k_{x}k_{y}\right]+h.c.\right\} ;$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 208}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,1}k_{y}\right)+c_{2}\sigma_{2}\left(k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+c_{2}\sigma_{2}\left(k_{z}-k_{x}\right)+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+c_{2}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left\{ \sigma_{+}\left[c_{2}\left(k_{x}^{2}-k_{y}^{2}\right)+ic_{3}k_{x}k_{y}\right]+h.c.\right\} ;$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left\{ \sigma_{+}\left[c_{2}\left(k_{x}^{2}-k_{y}^{2}\right)+ic_{3}k_{x}k_{y}\right]+h.c.\right\} ;$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 209}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(q_{x}^{2}+q_{y}^{2})+c_{3}q_{z}^{2}\right]\sigma_{0}+\left[c_{4}(q_{x}^{2}-q_{y}^{2})-c_{5}q_{x}q_{z}\right]\sigma_{3}+\left[(2c_{4}q_{x}q_{y}+c_{5}q_{y}q_{z}+ic_{6}q_{z})\sigma_{+}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{x}^{2}\right)\sigma_{0}+c_{6}\sigma_{3}k_{y}k_{z}+\left[\sigma_{+}\left(\alpha_{1}k_{x}+\alpha_{2}(k_{y}^{2}-k_{z}^{2})\right)+h.c.\right];$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,1}k_{y}\right)+c_{2}\sigma_{2}\left(k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+c_{2}\sigma_{2}\left(k_{z}-k_{x}\right)+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+c_{2}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}-c_{i,1}k_{z}\right)+\sum_{i=1}^{2}\sigma_{1}\left[c_{i,2}k_{x}+c_{i,3}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 210}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{6}\sigma_{2}k_{y}$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(q_{x}^{2}+q_{y}^{2})+c_{3}q_{z}^{2}\right]\sigma_{0}+\left[c_{4}(q_{x}^{2}-q_{y}^{2})-c_{5}q_{x}q_{z}\right]\sigma_{3}+\left[(2c_{4}q_{x}q_{y}+c_{5}q_{y}q_{z}+ic_{6}q_{z})\sigma_{+}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{x}+c_{3}\left[\sigma_{2}\left(k_{y}+k_{z}\right)+\sigma_{3}\left(k_{y}-k_{z}\right)\right];$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,1}k_{y}\right)+c_{2}\sigma_{2}\left(k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+c_{2}\sigma_{2}\left(k_{z}-k_{x}\right)+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+c_{2}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}-c_{i,1}k_{z}\right)+\sum_{i=1}^{2}\sigma_{1}\left[c_{i,2}k_{x}+c_{i,3}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG21.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 21}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 22}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 23}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 24}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline





\multicolumn{1}{l}{$W$;} & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 25}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{\sigma_{y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$H$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 26}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline



\multicolumn{1}{l}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline

\multicolumn{1}{l}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline


\multicolumn{1}{l}{$P$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{1,i}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{1,i}\sigma_{i}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{1,i}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{1,i}\sigma_{i}k_{z};$ \tabularnewline


\multicolumn{1}{l}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$H$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 27}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multicolumn{1}{l}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{6}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 28}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}00\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline



\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
$\Delta$;& &\tabularnewline




\multicolumn{1}{l}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multicolumn{1}{l}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 29}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline

\multicolumn{1}{l}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,1}k_{x}+c_{3}\Gamma_{0,3}k_{y}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\{R_{5},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,1}k_{x}+c_{3}\Gamma_{0,3}k_{y}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline


\multicolumn{1}{l}{$P$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 30}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}00\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline

\multicolumn{1}{l}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG211.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 211}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right)+c_{3}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)p_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)p_{y}\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sqrt{3}\sigma_{2}-\sigma_{1}\right)p_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)p_{y}\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)p_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)p_{y}\right];$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 212}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{C_{2a}|\frac{1}{4}\frac{3}{4}\frac{3}{4}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{4},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,2}q_{x}+\Gamma_{3,1}q_{y}-\Gamma_{3,3}q_{z}\right);$ \tabularnewline
 & $R_{8};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[\Gamma_{0,2}\left(k_{x}+k_{y}\right)+\Gamma_{3,3}\left(k_{x}-k_{y}\right)+\sqrt{2}\Gamma_{3,1}k_{z}\right];$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{4},R_{8}\};$  & $\left(c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{7}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}+c_{4}k_{z})\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}+c_{4}k_{z})\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{2}k_{x}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{2}k_{z}+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,0}k_{y}\right)+\left[k_{x}\left(\alpha\Gamma_{2,+}-c_{4}\Gamma_{2,3}\right)+k_{y}\left(\alpha\Gamma_{1,+}+c_{4}\Gamma_{1,3}\right)+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 213}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{C_{2a}|\frac{3}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{4},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,2}q_{x}+\Gamma_{3,1}q_{y}-\Gamma_{3,3}q_{z}\right);$ \tabularnewline
 & $R_{8};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[\Gamma_{0,2}\left(k_{x}+k_{y}\right)+\Gamma_{3,3}\left(k_{x}-k_{y}\right)+\sqrt{2}\Gamma_{3,1}k_{z}\right];$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{2},R_{6}\};$  & $\left(c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{7}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}+c_{4}k_{z})\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}+c_{4}k_{z})\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{2}k_{x}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{2}k_{z}+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,0}k_{y}\right)+\left[k_{x}\left(\alpha\Gamma_{2,+}-c_{4}\Gamma_{2,3}\right)+k_{y}\left(\alpha\Gamma_{1,+}+c_{4}\Gamma_{1,3}\right)+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 214}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{-}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{C_{2a}|\frac{1}{2}00\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sqrt{3}\sigma_{1}\left(k_{x}^{2}-k_{z}^{2}\right)+\sigma_{3}\left(k_{x}^{2}+k_{z}^{2}-2k_{y}^{2}\right)\right]+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{9};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}+A_{1}k_{y}+A_{2}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}+A_{1}k_{y}+A_{2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\left\{ q_{z}\sigma_{3}-\left[(-1)^{7/12}q_{+}\sigma_{-}+h.c.\right]\right\} ;$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}\left\{ q_{z}\sigma_{3}-\left[(-1)^{7/12}q_{+}\sigma_{-}+h.c.\right]\right\} ;$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\left\{ q_{z}\sigma_{3}-\left[(-1)^{7/12}q_{+}\sigma_{-}+h.c.\right]\right\} ;$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)p_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)p_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sqrt{3}\sigma_{2}-\sigma_{1}\right)p_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)p_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)p_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)p_{y}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 215}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{2}q_{z})\sigma_{0}+c_{3}\left(\sigma_{1}q_{y}-\sigma_{3}q_{x}\right);$ \tabularnewline


\multirow{1}{*}{$T$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{2}\left(k_{z}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y}+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left[\left(A_{6}-A_{4}\right)c_{5}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{5}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{5}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{5}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 216}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{3}\left[c_{4}\left(q_{x}^{2}-q_{y}^{2}\right)-c_{5}q_{x}q_{z}\right]+\left[\sigma_{+}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{2}q_{z})\sigma_{0}+c_{3}\left(\sigma_{1}q_{y}-\sigma_{3}q_{x}\right);$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{2}\left(k_{z}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y}+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 217}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q^{2}\right)\sigma_{0}+c_{3}\left[2\sigma_{1}q_{y}\left(q_{x}-\sqrt{2}q_{z}\right)+\sigma_{3}\left(2\sqrt{2}q_{x}q_{z}+q_{x}^{2}-q_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right);$ \tabularnewline


\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{2}q_{z})\sigma_{0}+c_{3}\left(\sigma_{1}q_{y}-\sigma_{3}q_{x}\right);$ \tabularnewline


\multirow{1}{*}{$F$;}&  $R_{3};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}+k_{z}\right)\right]\sigma_{0}+c_{3}\left[\sqrt{3}\sigma_{1}\left(k_{x}+k_{y}\right)+\sigma_{3}\left(k_{x}-k_{y}-2k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}+\left(A_{6}c_{4}-c_{7}A_{2}-2c_{5}A_{7}\right)\left(\sqrt{3}p_{x}-p_{y}\right)+\left[c_{6}A_{1}-A_{4}c_{4}+c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)\right]\left(p_{x}+\sqrt{3}p_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}+\left(A_{1}c_{6}-A_{4}c_{4}-2c_{5}A_{7}\right)\left(\sqrt{3}p_{x}-p_{y}\right)+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)-A_{6}c_{4}+A_{2}c_{6}\right]\left(p_{x}+\sqrt{3}p_{y}\right);$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 218}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $\{R_{5},R_{6}\};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\Gamma_{0,0}+c_{3}\left[\Gamma_{3,1}\left(k_{x}^{2}-k_{y}^{2}\right)-\frac{\Gamma_{3,2}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right]+\left\{ \alpha_{1}\left[\Gamma_{+,1}\left(k_{x}^{2}-k_{y}^{2}\right)-\frac{\Gamma_{+,2}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right]+h.c.\right\} ;$ \tabularnewline
 & $\{R_{9},R_{10}\};$  & $c_{1}S_{0,0}+c_{2}\left(S_{1,1}k_{x}+S_{1,2}k_{y}-S_{1,3}k_{z}\right)+c_{3}\left(S_{2,1}k_{x}+S_{2,2}k_{y}-S_{2,3}k_{z}\right)+c_{4}\left(S_{3,4}k_{x}-S_{3,6}k_{y}-S_{3,7}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+c_{3}(\sigma_{3}q_{x}-q_{y}\sigma_{1});$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]\sigma_{0}+c_{4}\sigma_{3}k_{y}+\left(c_{3}\sigma_{1}+c_{5}\sigma_{2}\right)\left(k_{x}-k_{z}\right);$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y}+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{3}k_{z}+\left[\left(A_{6}-A_{7}\right)c_{4}-\left(A_{2}+A_{3}\right)c_{5}\right]k_{x}-\left[\left(A_{6}+A_{7}\right)c_{4}+\left(A_{3}-A_{2}\right)c_{5}\right]k_{y};$ \tabularnewline
 & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{3}k_{z}+\left[\left(A_{6}+A_{7}\right)c_{4}+\left(A_{3}-A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{7}\right)c_{4}-\left(A_{2}+A_{3}\right)c_{5}\right]k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 219}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{3},R_{4}\};$  & $c_{2}\sigma_{3}q_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\sqrt{2}\Gamma_{0,3}q_{x}-\sqrt{2}\Gamma_{0,1}q_{y}+\Gamma_{3,0}q_{z}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}q_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{3}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}\left[\sigma_{3}q_{x}-q_{y}\left(\sigma_{-}+\sigma_{+}\right)\right];$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]\sigma_{0}+\sum_{i=1}^{3}\sigma_{i}\left[c_{i,1}k_{x}+c_{i,2}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{2}\left(k_{z}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y}+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 220}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{-}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{\sigma_{da}|\frac{1}{2}00\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\Gamma_{0,0}+c_{3}\left[\Gamma_{3,1}\left(k_{x}^{2}-k_{y}^{2}\right)-\frac{\Gamma_{3,2}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right]+\left\{ \alpha_{1}\left[\Gamma_{+,1}\left(k_{x}^{2}-k_{y}^{2}\right)-\frac{\Gamma_{+,2}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right]+h.c.\right\} ;$ \tabularnewline
 & $\{R_{9},R_{10}\};$  & $c_{1}S_{0,0}+c_{2}\left(S_{1,1}k_{x}+S_{1,2}k_{y}-S_{1,3}k_{z}\right)+c_{3}\left(S_{2,1}k_{x}+S_{2,2}k_{y}-S_{2,3}k_{z}\right)+c_{4}\left(S_{3,4}k_{x}-S_{3,6}k_{y}-S_{3,7}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{9};$  & $c_{1}\sigma_{0};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0};$ \tabularnewline
 & $R_{16};$  & $c_{1}\Gamma_{0,0}+\sqrt{6}\left(c_{2}-c_{3}\right)\left(\Gamma_{3,1}k_{y}+\Gamma_{3,2}k_{z}\right)+k_{x}\left[(3-i)c_{2}+4ic_{3}\right]\Gamma_{+,3}+\left(k_{y}\Gamma_{+,1}-k_{z}\Gamma_{+,2}\right)\left[\left(2ic_{2}+(3+i)c_{3}\right)\right];$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}\left[\sigma_{3}q_{x}-q_{y}\left(\sigma_{-}+\sigma_{+}\right)\right];$ \tabularnewline
\multirow{1}{*}{$D$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{2}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{3}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)\left(k_{x}+k_{y}\right)+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;}&  $R_{6};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}+k_{y}\right)+\frac{c_{3}\sigma_{3}\left(-k_{x}+k_{y}+2k_{z}\right)}{\sqrt{3}};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}+c_{5}\left[\left(p_{x}+\sqrt{3}p_{y}\right)\left(A_{5}-\sqrt{3}A_{8}\right)+2A_{7}\left(\sqrt{3}p_{x}-p_{y}\right)\right]+\left[\left(A_{4}+\sqrt{3}A_{6}\right)c_{4}-\left(A_{1}+\sqrt{3}A_{2}\right)c_{6}\right]p_{x}+\left[\left(\sqrt{3}A_{4}-A_{6}\right)c_{4}+\left(A_{2}-\sqrt{3}A_{1}\right)c_{6}\right]p_{y};$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}+c_{5}\left[\left(p_{x}+\sqrt{3}p_{y}\right)\left(A_{5}-\sqrt{3}A_{8}\right)+2A_{7}\left(\sqrt{3}p_{x}-p_{y}\right)\right]+\left[\left(\sqrt{3}A_{4}-A_{6}\right)c_{4}+\left(A_{2}-\sqrt{3}A_{1}\right)c_{6}\right]p_{x}-\left[\left(A_{4}+\sqrt{3}A_{6}\right)c_{4}-\left(A_{1}+\sqrt{3}A_{2}\right)c_{6}\right]p_{y}$\tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG221.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 221}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|000\},\{\sigma_{z}|000\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline


\multirow{1}{*}{$T$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 222}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{-}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{z}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2})\Gamma_{0,0}+\left[\alpha_{1}\Gamma_{+,0}\left(k_{x}^{2}-k_{z}^{2}\right)+\alpha_{2}k_{x}k_{z}\Gamma_{+,3}+\alpha_{3}k_{y}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\Gamma_{0,0}+\left(c_{3}\Gamma_{1,0}+c_{4}\Gamma_{2,0}\right)\left(2k_{x}^{2}-k_{y}^{2}-k_{z}^{2}\right)-\sqrt{3}\left(c_{3}\Gamma_{2,3}-c_{4}\Gamma_{1,3}\right)\left(k_{y}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{14};$  & $c_{1}S_{0,0}+c_{2}\left(k_{x}S_{1}^{\prime}+k_{y}S_{2}^{\prime}+k_{z}S_{3}^{\prime}\right)+c_{3}\left(k_{x}S_{4}^{\prime}+k_{y}S_{5}^{\prime}+k_{z}S_{6}^{\prime}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}\left(k_{x}-k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;}&  $R_{9};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+c_{6}\sigma_{2}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 &  & \tabularnewline
\multicolumn{3}{l}{Here, $S_{1}^{\prime}=3S_{0,1}-2S_{2,0}+2\sqrt{3}S_{2,8}-3S_{3,1}$,
$S_{2}^{\prime}=3\left(-S_{1,1}+S_{1,2}+S_{2,4}+S_{2,6}\right)$,
$S_{3}^{\prime}=3\left(S_{0,3}-S_{1,1}-S_{2,4}+S_{3,3}\right)$,}\tabularnewline
\multicolumn{3}{l}{$S_{4}^{\prime}=3\left(-S_{0,3}+S_{1,2}-S_{2,6}+S_{3,3}\right)$,
$S_{5}^{\prime}=-\left(3S_{1,3}+2S_{2,0}+3S_{2,5}+3S_{2,7}+\sqrt{3}S_{2,8}\right)$,
$S_{6}^{\prime}=\left(3S_{0,2}-2S_{2,0}+3S_{2,5}-\sqrt{3}S_{2,8}+3S_{3,2}\right)$.}\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right];$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right];$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 223}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|000\},\{\sigma_{z}|000\},\{C_{2c}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{12};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\Gamma_{0,0}+\left(c_{3}\Gamma_{1,0}+c_{4}\Gamma_{2,0}\right)\left(2k_{x}^{2}-k_{y}^{2}-k_{z}^{2}\right)-\sqrt{3}\left(c_{3}\Gamma_{2,3}-c_{4}\Gamma_{1,3}\right)\left(k_{y}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{14};$  & $c_{1}S_{0,0}+c_{2}\left(k_{x}S_{1}^{\prime}+k_{y}S_{2}^{\prime}+k_{z}S_{3}^{\prime}\right)+c_{3}\left(k_{x}S_{4}^{\prime}+k_{y}S_{5}^{\prime}+k_{z}S_{6}^{\prime}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}\left(k_{x}-k_{z}\right);$ \tabularnewline

\multirow{1}{*}{$T$;}&  $R_{10};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 &  & \tabularnewline
\multicolumn{3}{l}{Definition of $S_{i}^{\prime}$, see SG 222. }\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{9}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 224}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{-}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{z}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2c}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline

\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;}&  $R_{10};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+c_{6}\sigma_{2}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{5}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right];$\tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right];$\tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right];$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 225}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|000\},\{\sigma_{z}|000\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{5};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{1}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)-\sigma_{3}\left(c_{4}q_{x}^{2}-c_{4}q_{y}^{2}-c_{5}q_{x}q_{z}\right);$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{1}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)+\sigma_{3}\left(c_{4}q_{x}^{2}-c_{4}q_{y}^{2}-c_{5}q_{x}q_{z}\right);$ \tabularnewline
\multirow{1}{*}{$W$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]+\sigma_{3}c_{3}\left(k_{y}-k_{z}\right)+\sigma_{1}\left[c_{4}k_{x}+c_{5}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 226}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{-}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{z}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,1}q_{x}+\Gamma_{0,2}q_{y}\right)+q_{z}\left(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}q_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{13},R_{16}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\{R_{14},R_{15}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $R_{20};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{x}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{y}+k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 227}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{-}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\{\sigma_{x}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\{\sigma_{z}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\{C_{2c}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{5};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{1}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)-\sigma_{3}\left(c_{4}q_{x}^{2}-c_{4}q_{y}^{2}-c_{5}q_{x}q_{z}\right);$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{1}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)+\sigma_{3}\left(c_{4}q_{x}^{2}-c_{4}q_{y}^{2}-c_{5}q_{x}q_{z}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{y}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $R_{12};$  & $c_{1}\sigma_{0}+c_{2}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{y}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]+\sigma_{3}c_{3}\left(k_{y}-k_{z}\right)+\sigma_{1}\left[c_{4}k_{x}+c_{5}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 228}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{-}|\frac{3}{4}\frac{3}{4}\frac{3}{4}\},\{\sigma_{x}|\frac{3}{4}\frac{3}{4}\frac{3}{4}\},\{\sigma_{z}|\frac{3}{4}\frac{3}{4}\frac{3}{4}\},\{C_{2c}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,1}q_{x}+\Gamma_{0,2}q_{y}\right)+q_{z}\left(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}q_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{13},R_{14}\};$  & $c_{1}\Gamma_{0,0}+c_{3}\Gamma_{0,1}\left(k_{y}+k_{z}\right)-c_{3}\Gamma_{3,2}\left(k_{y}-k_{z}\right)+\left[\alpha_{1}k_{x}\Gamma_{+,1}-i\alpha_{2}\Gamma_{+,0}\left(k_{y}-k_{z}\right)+\alpha_{2}\Gamma_{+,3}\left(k_{y}+k_{z}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{4},R_{8}\};$  & $\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{x}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{y}+k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 229}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|000\},\{\sigma_{z}|000\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right);$ \tabularnewline


\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline


\multirow{1}{*}{$F$;}&  $R_{3};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}+k_{y}\right)+\frac{c_{3}\sigma_{3}\left(k_{x}-k_{y}-2k_{z}\right)}{\sqrt{3}};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{3}+c_{4}p_{z}\right)+c_{5}\left[\left(A_{5}-\sqrt{3}A_{8}\right)\left(p_{x}+\sqrt{3}p_{y}\right)+2A_{7}\left(p_{y}-\sqrt{3}p_{x}\right)\right]+c_{6}\left[\left(A_{1}-\sqrt{3}A_{2}\right)p_{x}+\left(\sqrt{3}A_{1}+A_{2}\right)p_{y}\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{3}+c_{4}p_{z}\right)+c_{5}\left[\left(A_{5}-\sqrt{3}A_{8}\right)\left(p_{x}+\sqrt{3}p_{y}\right)+2A_{7}\left(p_{y}-\sqrt{3}p_{x}\right)\right]+c_{6}\left[A_{2}\left(p_{x}+\sqrt{3}p_{y}\right)+A_{1}\left(\sqrt{3}p_{x}-p_{y}\right)\right];$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 230}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}0\},\{\sigma_{z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2c}|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)\left(k_{x}^{2}-k_{z}^{2}\right)\left(k_{y}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left(c_{1}+c_{2}q^{2}\right)\Gamma_{0,0}+\left[i\alpha_{1}\Gamma_{+,0}\left(q_{x}^{2}-q_{y}^{2}+2\sqrt{2}q_{x}q_{z}\right)+2\alpha_{1}q_{y}\Gamma_{+,3}\left(q_{x}-\sqrt{2}q_{z}\right)+h.c.\right];$ \tabularnewline
 & $R_{14};$  & $c_{1}S_{0,0}+c_{2}\left(S_{2,3}k_{x}+S_{2,1}k_{y}+S_{2,2}k_{z}\right)+c_{3}\left(S_{3,7}k_{x}+S_{3,4}k_{y}-S_{3,6}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+\left[\alpha_{1}\left(q_{x}^{\prime}\Gamma_{+,0}-iq_{y}^{\prime}\Gamma_{+,3}+iq_{z}^{\prime}\Gamma_{+,1}\right)+h.c.\right];$ \tabularnewline
 & $R_{16};$  & $c_{1}\Gamma_{0,0}+(c_{2}-c_{3})\left(\Gamma_{3,2}k_{z}+\Gamma_{3,1}k_{y}\right)++\left\{ \left[2ic_{2}+(3+i)c_{3}\right]\left(k_{y}\Gamma_{+,1}-k_{z}\Gamma_{+,2}\right)+\left[(3-i)c_{2}+4ic_{3}\right]k_{x}\Gamma_{+,3}+h.c.\right\} ;$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline
\multirow{1}{*}{$D$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}-k_{y}\right)+c_{4}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;}&  $R_{6};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}+k_{y}\right)-\frac{c_{3}\sigma_{3}\left(k_{x}-k_{y}-2k_{z}\right)}{\sqrt{3}};$ \tabularnewline
 &  & \tabularnewline
\multicolumn{3}{l}{Here, $\left\{ q_{x}^{\prime},q_{y}^{\prime},q_{z}^{\prime}\right\} =\left\{ \left(1+\sqrt{3}\right)k_{x}-2k_{y}+\left(\sqrt{3}-1\right)k_{z},\left(1-\sqrt{3}\right)k_{x}-2k_{y}-\left(1+\sqrt{3}\right)k_{z},-2k_{x}-2k_{y}+2k_{z}\right\} $.}\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{3}p_{z}\right)+c_{4}\left[\left(A_{5}-\sqrt{3}A_{8}\right)\left(p_{x}+\sqrt{3}p_{y}\right)+2A_{7}\left(\sqrt{3}p_{x}-p_{y}\right)\right]+c_{5}\left[\left(A_{1}+\sqrt{3}A_{2}\right)p_{x}+\left(\sqrt{3}A_{1}-A_{2}\right)p_{y}\right]$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{3}+c_{4}p_{z}\right)+c_{5}\left[\left(A_{5}-\sqrt{3}A_{8}\right)\left(p_{x}+\sqrt{3}p_{y}\right)+2A_{7}\left(\sqrt{3}p_{x}-p_{y}\right)\right]+c_{6}\left[A_{2}\left(p_{x}+\sqrt{3}p_{y}\right)+A_{1}\left(p_{y}-\sqrt{3}p_{x}\right)\right]$\tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG31.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 31}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline

\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 32}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}\frac{1}{2}0\},\{\sigma_{y}|0\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 33}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,1}k_{x}+c_{3}\Gamma_{0,3}k_{y}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 34}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}\frac{1}{2}0\},\{\sigma_{y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 35}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{6}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{6}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 36}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|00\frac{1}{2}\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline



\multirow{1}{*}{$A$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$H$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 37}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline





\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$H$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 38}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2y}|000\},\{\sigma_{x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
$\Delta$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$B$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$F$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 39}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2y}|000\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i}$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
$\Delta$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$B$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$F$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 40}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2y}|000\},\{\sigma_{x}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline





\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
$\Delta$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$F$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG41.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 41}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2y}|000\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 42}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 43}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|00\frac{1}{2}\},\{\sigma_{y}|\frac{1}{2}00\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline


\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 44}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 45}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{y}+c_{3}k_{z})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$W$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline





\multirow{1}{*}{$D$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 46}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{\sigma_{y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{y}+c_{3}k_{z})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}+c_{2}\sigma_{3}k_{z};$ \tabularnewline





\multirow{1}{*}{$D$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 47}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 48}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\left(c_{1}+c_{2}k_{x}\right)+\sigma_{3}\left(c_{3}+c_{4}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\left(c_{1}+c_{2}k_{x}\right)+\sigma_{3}\left(c_{3}+c_{4}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\left(c_{1}+c_{2}k_{x}\right)+\sigma_{3}\left(c_{3}+c_{4}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\left(c_{1}+c_{2}k_{x}\right)+\sigma_{3}\left(c_{3}+c_{4}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 49}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 50}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG51.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 51}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 52}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+c_{3}\Gamma_{3,1}k_{y}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 53}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\{I|\frac{1}{2}00\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}-c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}-c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 54}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\{I|0\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+c_{3}\Gamma_{3,1}k_{y}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+c_{3}\Gamma_{3,1}k_{y}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $R_{5};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 55}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline


\multirow{1}{*}{$C$;} & $\{R_{2},R_{4}\};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline


\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{2}k_{z}+c_{1})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y}$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{2}k_{z}+c_{1})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{1,1}+c_{5}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 56}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{x}+c_{2}\Gamma_{0,2}k_{y}+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y}+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{2}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{2}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y}$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{2}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{3},R_{4}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\left[\Gamma_{i,0}c_{i,1}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\left[\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{1,1}+c_{5}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 57}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|0\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2})k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2})k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline


\multirow{1}{*}{$C$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{2}+c_{4}\sigma_{1})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{2}+c_{4}\sigma_{1})k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{2}+c_{4}\sigma_{1})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{2}+c_{4}\sigma_{1})k_{y};$ \tabularnewline


\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{5}k_{z})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,2}k_{x}+c_{i,2}\Gamma_{i,1}k_{y});$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 58}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{y}+c_{3}\sigma_{1}k_{z})k_{x};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{y}+c_{3}\sigma_{1}k_{z})k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y}$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y}$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{1,1}+c_{5}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 59}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline


\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline


\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{3},R_{4}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y}$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{1,1}+c_{5}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 60}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}0\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{y}+c_{3}\sigma_{1}k_{z})k_{x};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{y}+c_{3}\sigma_{1}k_{z})k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y}+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{x}+c_{2}\Gamma_{0,2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{5}k_{z})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,1}k_{x}+c_{i,2}\Gamma_{i,2}k_{y});$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{5}\right\} ,\left\{ R_{5}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{x}+\Gamma_{1,0}\left(c_{2}+c_{3}k_{x}\right)+\left(c_{4}\Gamma_{0,3}+c_{5}\Gamma_{1,3}+c_{6}\Gamma_{3,3}\right)k_{y}+c_{7}\Gamma_{2,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\left[\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG61.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 61}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2})k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+(c_{2}\Gamma_{1,2}+c_{3}\Gamma_{2,2})k_{y}+c_{4}\Gamma_{0,2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+(c_{2}\Gamma_{1,2}+c_{3}\Gamma_{2,2})k_{x}+c_{4}\Gamma_{0,2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\Gamma_{0,0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,3}k_{x}k_{y}+\sum_{i=1}^{3}(c_{i,2}\Gamma_{i,1}k_{x}k_{z}+c_{i,3}\Gamma_{i,2}k_{y}k_{z});$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\Gamma_{0,0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,3}k_{x}k_{y}+\sum_{i=1}^{3}(c_{i,2}\Gamma_{i,1}k_{x}k_{z}+c_{i,3}\Gamma_{i,2}k_{y}k_{z});$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{2}k_{y})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,3}k_{x}+c_{i,2}\Gamma_{i,1}k_{z});$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{2}k_{x})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,1}k_{y}+c_{i,2}\Gamma_{i,3}k_{z});$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{2}k_{z})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,1}k_{x}+c_{i,2}\Gamma_{i,3}k_{y});$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & \multicolumn{1}{l}{$\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$ } & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 62}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z}$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z}$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z}$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z}$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{2}\sigma_{3}k_{y}k_{z}$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{2}\sigma_{3}k_{y}k_{z}$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{3}\Gamma_{3,1}k_{x}+(c_{4}\Gamma_{1,2}+c_{2}\Gamma_{2,2})k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{3,1}k_{x}+c_{3}\Gamma_{0,2}k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{z};$ \tabularnewline
 & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}k_{z};$ \tabularnewline
 & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{2}k_{z})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,3}k_{x}+c_{i,2}\Gamma_{i,1}k_{y});$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{z}\left(c_{4}\Gamma_{1,0}+c_{5}\Gamma_{2,3}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{z}\left(c_{4}\Gamma_{1,0}+c_{5}\Gamma_{2,3}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 63}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|00\frac{1}{2}\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline



\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 64}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|00\frac{1}{2}\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{4}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{4}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 65}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 66}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline





\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{4}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2}+c_{4}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 67}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 68}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{4}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{4}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 69}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 70}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline


\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG71.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 71}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sigma_{1}\left(c_{5}k_{y}+c_{6}k_{z}\right);$ \tabularnewline
$\Delta$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sigma_{1}\left(c_{5}k_{x}+c_{6}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 72}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{y}+c_{3}k_{z})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{z};$ \tabularnewline





\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 73}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{y}+c_{3}k_{z})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{9},R_{9}\};$  & $2c_{1}\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,2}k_{x}+c_{i,2}\Gamma_{i,3}k_{y}+c_{i,3}\Gamma_{i,1}k_{z});$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 74}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x}+c_{3}\sigma_{3}k_{y};$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sigma_{1}\left(c_{5}k_{y}+c_{6}k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sigma_{1}\left(c_{5}k_{x}+c_{6}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 75}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline











\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 76}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{4}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 77}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline











\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 78}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{3}{4}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 79}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})+c_{i,3}k_{z}\right]\sigma_{i};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 80}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+c_{3}(\sigma_{2}k_{x}+\sigma_{1}k_{y})+c_{4}(\sigma_{1}k_{x}-\sigma_{2}k_{y})+c_{2}\sigma_{3}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG81.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 81}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left(A_{4}c_{3}+A_{6}c_{4}-A_{1}c_{6}-A_{2}c_{7}\right)k_{x}+\left(-A_{6}c_{3}+A_{4}c_{4}-A_{2}c_{6}+A_{1}c_{7}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left(A_{4}c_{3}+A_{6}c_{4}-A_{1}c_{6}-A_{2}c_{7}\right)k_{x}+\left(-A_{6}c_{3}+A_{4}c_{4}-A_{2}c_{6}+A_{1}c_{7}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 82}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left(A_{4}c_{3}+A_{6}c_{4}-A_{1}c_{6}-A_{2}c_{7}\right)k_{x}+\left(-A_{6}c_{3}+A_{4}c_{4}-A_{2}c_{6}+A_{1}c_{7}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left(A_{4}c_{3}+A_{6}c_{4}-A_{1}c_{6}-A_{2}c_{7}\right)k_{x}+\left(-A_{6}c_{3}+A_{4}c_{4}-A_{2}c_{6}+A_{1}c_{7}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 83}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{I|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 84}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 85}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{7}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline




\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{2}-A_{3}\right)c_{4}\right]k_{x}+\left[\left(A_{3}-A_{2}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 86}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{7}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline




\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{2}-A_{3}\right)c_{4}\right]k_{x}+\left[\left(A_{3}-A_{2}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 87}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{I|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})+c_{i,3}k_{z}\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 88}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\{I|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{4}\};$  & $c_{2}(\sigma_{2}k_{x}+\sigma_{1}k_{y})+c_{3}(\sigma_{1}k_{x}+\sigma_{2}k_{y})+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{2}(\sigma_{2}k_{x}+\sigma_{1}k_{y})+c_{3}(\sigma_{1}k_{x}+\sigma_{2}k_{y})+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{7}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{4}k_{x}+c_{3}k_{y})\sigma_{1}+(c_{6}k_{x}+c_{5}k_{y})\sigma_{2};$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 89}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline











\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 90}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline



\multirow{1}{*}{$V$;} & $\{R_{1},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+\left\{ (1+i)\left[\left(c_{4}\Gamma_{+,0}+ic_{5}\Gamma_{+,3}\right)k_{-}+ik_{+}\left(c_{6}\Gamma_{+,1}+c_{7}\Gamma_{+,2}\right)\right]+h.c.\right\} ;$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> basicinfo/merge/mergeSG91.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 91}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{4}\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 92}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{4}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{6},R_{7}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[\Gamma_{0,2}(k_{x}-k_{y})+\Gamma_{3,3}(k_{x}+k_{y})\right]+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+\left\{ (1+i)\left[\left(c_{4}\Gamma_{+,0}+ic_{5}\Gamma_{+,3}\right)k_{-}+ik_{+}\left(c_{6}\Gamma_{+,1}+c_{7}\Gamma_{+,2}\right)\right]+h.c.\right\} ;$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+\Gamma_{3,0}c_{3}k_{x}+c_{4}\Gamma_{1,0}k_{z}+c_{5}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{2,i}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 93}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline











\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 94}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline



\multirow{1}{*}{$V$;} & $\{R_{1},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+\left\{ (1+i)\left[\left(c_{4}\Gamma_{+,0}+ic_{5}\Gamma_{+,3}\right)k_{-}+ik_{+}\left(c_{6}\Gamma_{+,1}+c_{7}\Gamma_{+,2}\right)\right]+h.c.\right\} ;$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 95}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{3}{4}\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 96}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{3}{4}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{6},R_{7}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[\Gamma_{0,2}(k_{x}-k_{y})+\Gamma_{3,3}(k_{x}+k_{y})\right]+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+\left\{ (1+i)\left[\left(c_{4}\Gamma_{+,0}+ic_{5}\Gamma_{+,3}\right)k_{-}+ik_{+}\left(c_{6}\Gamma_{+,1}+c_{7}\Gamma_{+,2}\right)\right]+h.c.\right\} ;$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+\Gamma_{3,0}c_{3}k_{x}+c_{4}\Gamma_{1,0}k_{z}+c_{5}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{2,i}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 97}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}k_{y}+c_{i,2}k_{z})\sigma_{i}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 98}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\{C_{2x}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{2}k_{x}-\sigma_{3}k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 99}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$\tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 100}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{5}\sigma_{2})k_{y}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{5}\sigma_{2})k_{y}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$\tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/a <==
mergeSG1.tex
20
True
False
[]
True
False
[]
True
False
['\\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\\tabularnewline\n\\multicolumn{3}{l}{ }\\tabularnewline\n\\multirow{1}{*}{$\\Lambda$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$V$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$W$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$U$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline']
True
False
['\\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\\tabularnewline\n\\multicolumn{3}{l}{ }\\tabularnewline\n\\multirow{1}{*}{$\\Lambda$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$V$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$W$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$U$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline']
True
False
['\\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\\tabularnewline\n\\multicolumn{3}{l}{ }\\tabularnewline\n\\multirow{1}{*}{$\\Lambda$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$U$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sum_{i=1}^{2}\\sigma_{i}\\left(c_{i,1}k_{x}+c_{i,2}k_{y}\\right);$ \\tabularnewline']
True
False
[]
True
False
[]
True
False
[]
True
False
[]
True
False
['\\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\\tabularnewline\n\\multicolumn{3}{l}{ }\\tabularnewline\n\\multirow{1}{*}{$\\Lambda$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sigma_{1}\\left(c_{4}k_{x}+c_{5}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$V$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sigma_{1}\\left(c_{4}k_{x}+c_{5}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$W$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sigma_{1}\\left(c_{4}k_{x}+c_{5}k_{y}\\right);$ \\tabularnewline', '\\multirow{1}{*}{$U$;} & $\\left\\{ R_{1}\\right\\} ,\\left\\{ R_{2}\\right\\} ;$  & $\\sigma_{0}\\left(c_{1}+c_{2}k_{z}\\right)+c_{3}\\sigma_{3}k_{z}+\\sigma_{1}\\left(c_{4}k_{x}+c_{5}k_{y}\\right);$ \\tabularnewline']


==> dSG/basicinfo/merge/mergeSG1.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 1}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{t}$; $\{E|000\},\mathcal{T}$; Non-Centrosymmetric; without
SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 2}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{t}$; $\{I|000\},\mathcal{T}$; Centrosymmetric; without
SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 3}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 4}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|00\frac{1}{2}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 5}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{C_{2z}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 6}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{\sigma_{z}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 7}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{\sigma_{z}|\frac{1}{2}00\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multicolumn{1}{l}{$B$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline



\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 8}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{\sigma_{z}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 9}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{\sigma_{z}|\frac{1}{2}00\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$M$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline



\multirow{1}{*}{$U$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{l||l||l||l||l||l||l||l||ll}

\hline
\multicolumn{9}{l}{Symmetry-protected accidental points at high symmetry line} & \tabularnewline
\multicolumn{9}{l}{ } & \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 10}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|000\},\{I|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG101.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 101}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline



\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 102}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{3}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}-\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}-\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 103}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,3}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,3}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 104}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,3}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{3}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}-\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}-\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 105}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 106}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,3}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{3}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}-\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}-\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 107}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 108}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$N$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 109}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}(k_{x}+k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\left[(\sigma_{1}-\sigma_{3})k_{x}+(\sigma_{1}+\sigma_{3})k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{2}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{2}(k_{x}-k_{y});$ \tabularnewline




\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $[c_{1}+c_{2}(k_{x}-k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}+k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{4}c_{3}+A_{1}c_{4}\right)k_{x}+\left(A_{6}c_{4}-A_{2}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{4}\right)k_{x}+\left(A_{2}c_{3}+A_{6}c_{4}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{4}\right)k_{x}+\left(A_{1}c_{3}+A_{4}c_{4}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{6}c_{3}+A_{2}c_{4}\right)k_{x}+\left(A_{4}c_{4}-A_{1}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 110}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$N$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}(k_{x}+k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{10},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[(k_{x}+k_{y})\Gamma_{0,1}+(k_{x}-k_{y})\Gamma_{0,3}\right]+\sum_{i=1}^{3}c_{i,1}\left[(k_{x}+k_{y})\Gamma_{i,1}-(k_{x}-k_{y})\Gamma_{i,3}+k_{z}\Gamma_{i,0}\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}k_{x}k_{y}\sigma_{2}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(k_{x}+k_{y})\sigma_{1}+c_{4}(k_{x}-k_{y})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $[c_{1}+c_{2}(k_{x}+k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $[c_{1}+c_{2}(k_{x}-k_{y})]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}+k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{4}c_{3}+A_{1}c_{4}\right)k_{x}+\left(A_{6}c_{4}-A_{2}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{4}\right)k_{x}+\left(A_{2}c_{3}+A_{6}c_{4}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{4}\right)k_{x}+\left(A_{1}c_{3}+A_{4}c_{4}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left(A_{6}c_{3}+A_{2}c_{4}\right)k_{x}+\left(A_{4}c_{4}-A_{1}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG11.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 11}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|00\frac{1}{2}\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 12}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{C_{2z}|000\},\{I|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 13}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|000\},\{I|\frac{1}{2}00\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$B$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline



\multirow{1}{*}{$D$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 14}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}$; $\{C_{2z}|00\frac{1}{2}\},\{I|\frac{1}{2}0\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multicolumn{1}{l}{}& &\tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline

\multicolumn{1}{l}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\{R_{2},R_{4}\};$  & $h+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $h+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{2},R_{4}\};$  & $h+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $h+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
 &  & \tabularnewline
\multicolumn{3}{l}{Here, $h=(c_{1}+c_{2}k_{x}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}k_{y}+c_{5}k_{z}^{2})\sigma_{0}$.}\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 15}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{m}^{b}$; $\{C_{2z}|000\},\{I|\frac{1}{2}00\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$A$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$M$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline



\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y});$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 16}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
















$\Lambda$;& &\tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 17}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline



\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

$D$;& &\tabularnewline
\multicolumn{1}{l}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline


\multicolumn{1}{l}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 18}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multicolumn{1}{l}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
$R$;  & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multicolumn{1}{l}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline


\multicolumn{1}{l}{$C$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline


\multicolumn{1}{l}{$H$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+c_{4}\Gamma_{1,0}k_{y}+c_{5}\Gamma_{2,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}k_{x}\Gamma_{1,i}+c_{i,2}k_{y}\Gamma_{2,i}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 19}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\{R_{5},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,3}k_{x}+c_{3}\Gamma_{0,1}k_{y}+c_{4}\Gamma_{0,2}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}-c_{4}\sigma_{2})k_{z};$ \tabularnewline
$\Sigma$;& &\tabularnewline
\multicolumn{1}{l}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multicolumn{1}{l}{$H$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{y};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{x}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{2,0}k_{x}+c_{5}\Gamma_{1,0}k_{z}+\sum_{i=1}^{3}\left(c_{i,1}k_{x}\Gamma_{1,i}+c_{i,2}k_{z}\Gamma_{2,i}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{1,0}k_{y}+c_{5}\Gamma_{2,0}k_{z}+\sum_{i=1}^{3}\left(c_{i,1}k_{z}\Gamma_{1,i}+c_{i,2}k_{y}\Gamma_{2,i}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+c_{4}\Gamma_{1,0}k_{y}+c_{5}\Gamma_{2,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}k_{x}\Gamma_{1,i}+c_{i,2}k_{y}\Gamma_{2,i}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 20}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline


\multicolumn{1}{l}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline



\multicolumn{1}{l}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

$\Delta$;& &\tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multicolumn{1}{l}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG111.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 111}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2x}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 112}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2x}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(4_{3}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(4_{3}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(4_{3}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(4_{3}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 113}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{3},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{x}k_{y};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{2,1}+c_{3}\Gamma_{2,2}\right)+c_{4}\left(\Gamma_{1,0}k_{x}+\Gamma_{1,3}k_{y}\right)+c_{5}\left(\Gamma_{2,3}k_{x}+\Gamma_{2,0}k_{y}\right)-k_{y}\left(c_{6}\Gamma_{1,1}-c_{7}\Gamma_{1,2}\right);$ \tabularnewline
 & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}-c_{3}\Gamma_{1,2}\right)+c_{4}\left(\Gamma_{1,3}k_{x}-\Gamma_{1,0}k_{y}\right)+c_{5}\left(\Gamma_{2,3}k_{y}-\Gamma_{2,0}k_{x}\right)+k_{y}\left(c_{6}\Gamma_{2,1}+c_{7}\Gamma_{2,2}\right);$ \tabularnewline
 & $\left\{ R_{3},R_{3}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{0,3}+c_{3}\Gamma_{3,3}\right)k_{x}k_{y}+\left(c_{4}\Gamma_{1,3}+c_{5}\Gamma_{2,0}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 114}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,2}k_{z}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,1}(k_{x}^{2}-k_{y}^{2})+c_{i,2}\Gamma_{i,2}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{3},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{x}k_{y};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{2,1}+c_{3}\Gamma_{2,2}\right)+c_{4}\left(\Gamma_{1,0}k_{x}+\Gamma_{1,3}k_{y}\right)+c_{5}\left(\Gamma_{2,3}k_{x}+\Gamma_{2,0}k_{y}\right)-k_{y}\left(c_{6}\Gamma_{1,1}-c_{7}\Gamma_{1,2}\right);$ \tabularnewline
 & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}-c_{3}\Gamma_{1,2}\right)+c_{4}\left(\Gamma_{1,3}k_{x}-\Gamma_{1,0}k_{y}\right)+c_{5}\left(\Gamma_{2,3}k_{y}-\Gamma_{2,0}k_{x}\right)+k_{y}\left(c_{6}\Gamma_{2,1}+c_{7}\Gamma_{2,2}\right);$ \tabularnewline
 & $\left\{ R_{3},R_{3}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{0,3}+c_{3}\Gamma_{3,3}\right)k_{x}k_{y}+\left(c_{4}\Gamma_{1,3}+c_{5}\Gamma_{2,0}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 115}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2a}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 116}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2a}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline



\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 117}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2a}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 118}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\{C_{2a}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 119}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\{C_{2a}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 120}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\{C_{2a}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$N$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{1};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{3}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}(k_{x}^{2}-k_{y}^{2})+(c_{6}\sigma_{1}+c_{7}\sigma_{2})k_{x}k_{y};$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}-\left(A_{6}c_{3}+A_{2}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{4}c_{3}+A_{1}c_{5}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG121.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 121}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}k_{z}+c_{5}k_{x}k_{y})\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 122}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\{C_{2x}|\frac{1}{4}\frac{3}{4}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}(k_{x}+k_{y});$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{y}+\sigma_{2}k_{x});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{y}+\sigma_{2}k_{x});$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+(c_{6}\sigma_{1}+c_{7}\sigma_{2})(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{2}(k_{x}-k_{y});$ \tabularnewline




\multirow{1}{*}{$U$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}-k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}-k_{y})\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})(k_{x}+k_{y})+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{3}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 123}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 124}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{3}\sigma_{2}(k_{x}-k_{y})+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 125}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{2}(k_{x}^{2}-k_{y}^{2})+c_{6}\sigma_{3}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 126}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{2}(k_{x}^{2}-k_{y}^{2})+c_{6}\sigma_{3}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{2}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 127}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left(c_{2}\Gamma_{1,0}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}+c_{3}\Gamma_{2,3}\right)\left(k_{x}-k_{y}\right)-\left(c_{3}\Gamma_{1,0}-c_{3}\Gamma_{1,3}+c_{2}\Gamma_{2,0}-c_{2}\Gamma_{2,3}\right)\left(k_{x}+k_{y}\right)+\left[(1+i)\left(c_{3}+ic_{2}\right)\left(\Gamma_{2,+}k_{+}+\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
 & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{7},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right)k_{x}k_{y};$\tabularnewline
 & $\left\{ R_{7},R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left[c_{2}\left(\Gamma_{1,0}+\Gamma_{1,3}\right)-c_{3}\left(\Gamma_{2,0}+\Gamma_{2,3}\right)\right]\left(k_{x}+k_{y}\right)+\left[c_{2}\left(\Gamma_{2,0}-\Gamma_{2,3}\right)-c_{3}\left(\Gamma_{1,0}-\Gamma_{1,3}\right)\right]\left(k_{x}-k_{y}\right)+\left[(1+i)\left(c_{2}+ic_{3}\right)\left(\Gamma_{2,+}k_{+}-\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{0,1}+c_{3}\Gamma_{0,2}+c_{4}\Gamma_{3,1}+c_{5}\Gamma_{3,2}\right)+k_{z}\left(c_{6}\Gamma_{1,0}+c_{7}\Gamma_{2,3}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{0,1}+c_{3}\Gamma_{0,2}+c_{4}\Gamma_{3,1}+c_{5}\Gamma_{3,2}\right)+k_{z}\left(c_{6}\Gamma_{1,0}+c_{7}\Gamma_{2,3}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 128}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,2}k_{z}+\sum_{i=1}^{2}\left[c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{2}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left(c_{2}\Gamma_{1,0}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}+c_{3}\Gamma_{2,3}\right)\left(k_{x}-k_{y}\right)-\left(c_{3}\Gamma_{1,0}-c_{3}\Gamma_{1,3}+c_{2}\Gamma_{2,0}-c_{2}\Gamma_{2,3}\right)\left(k_{x}+k_{y}\right)+\left[(1+i)\left(c_{3}+ic_{2}\right)\left(\Gamma_{2,+}k_{+}+\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
 & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{7},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right)k_{x}k_{y};$\tabularnewline
 & $\left\{ R_{7},R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left[c_{2}\left(\Gamma_{1,0}+\Gamma_{1,3}\right)-c_{3}\left(\Gamma_{2,0}+\Gamma_{2,3}\right)\right]\left(k_{x}+k_{y}\right)+\left[c_{2}\left(\Gamma_{2,0}-\Gamma_{2,3}\right)-c_{3}\left(\Gamma_{1,0}-\Gamma_{1,3}\right)\right]\left(k_{x}-k_{y}\right)+\left[(1+i)\left(c_{2}+ic_{3}\right)\left(\Gamma_{2,+}k_{+}-\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{0,1}+c_{3}\Gamma_{0,2}+c_{4}\Gamma_{3,1}+c_{5}\Gamma_{3,2}\right)+k_{z}\left(c_{6}\Gamma_{1,0}+c_{7}\Gamma_{2,3}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 129}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}+\Gamma_{1,2}+\Gamma_{2,1}-\Gamma_{2,2}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}-\Gamma_{1,2}+\Gamma_{2,1}+\Gamma_{2,2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right]$\tabularnewline
 & $\left\{ R_{2},R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,1}-\Gamma_{1,2}-\Gamma_{2,1}+\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,1}+\Gamma_{1,2}-\Gamma_{2,1}-\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 130}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{9},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,1}k_{z}+c_{5}\Gamma_{0,3}(k_{x}^{2}-k_{y}^{2})+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{13},R_{14}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,3}(k_{x}^{2}-k_{y}^{2})+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,3}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{3,1}k_{x}+c_{3}\Gamma_{0,2}k_{z}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{2}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}+\Gamma_{1,2}+\Gamma_{2,1}-\Gamma_{2,2}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}-\Gamma_{1,2}+\Gamma_{2,1}+\Gamma_{2,2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right]$\tabularnewline
 & $\left\{ R_{2},R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,1}-\Gamma_{1,2}-\Gamma_{2,1}+\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,1}+\Gamma_{1,2}-\Gamma_{2,1}-\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG131.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 131}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 132}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|000\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline



\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 133}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,3}k_{x}k_{y}+c_{4}\Gamma_{i,0}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{2}(k_{x}^{2}-k_{y}^{2})+c_{6}\sigma_{3}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 134}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{2}(k_{x}^{2}-k_{y}^{2})+c_{6}\sigma_{3}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $c_{3}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right]+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 135}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{9},R_{10}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,1}k_{z}+c_{5}\Gamma_{0,3}(k_{x}^{2}-k_{y}^{2})+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{13},R_{14}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,3}(k_{x}^{2}-k_{y}^{2})+\sum_{i=1}^{2}\left[c_{i,1}\Gamma_{i,2}k_{z}+c_{i,2}\Gamma_{i,3}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left(c_{2}\Gamma_{1,0}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}+c_{3}\Gamma_{2,3}\right)\left(k_{x}-k_{y}\right)-\left(c_{3}\Gamma_{1,0}-c_{3}\Gamma_{1,3}+c_{2}\Gamma_{2,0}-c_{2}\Gamma_{2,3}\right)\left(k_{x}+k_{y}\right)+\left[(1+i)\left(c_{3}+ic_{2}\right)\left(\Gamma_{2,+}k_{+}+\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
 & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{7},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right)k_{x}k_{y};$\tabularnewline
 & $\left\{ R_{7},R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left[c_{2}\left(\Gamma_{1,0}+\Gamma_{1,3}\right)-c_{3}\left(\Gamma_{2,0}+\Gamma_{2,3}\right)\right]\left(k_{x}+k_{y}\right)+\left[c_{2}\left(\Gamma_{2,0}-\Gamma_{2,3}\right)-c_{3}\left(\Gamma_{1,0}-\Gamma_{1,3}\right)\right]\left(k_{x}-k_{y}\right)+\left[(1+i)\left(c_{2}+ic_{3}\right)\left(\Gamma_{2,+}k_{+}-\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 136}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left(c_{2}\Gamma_{1,0}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}+c_{3}\Gamma_{2,3}\right)\left(k_{x}-k_{y}\right)-\left(c_{3}\Gamma_{1,0}-c_{3}\Gamma_{1,3}+c_{2}\Gamma_{2,0}-c_{2}\Gamma_{2,3}\right)\left(k_{x}+k_{y}\right)+\left[(1+i)\left(c_{3}+ic_{2}\right)\left(\Gamma_{2,+}k_{+}+\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
 & $\left\{ R_{5},R_{6}\right\} ,\left\{ R_{7},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)\left(k_{x}^{2}-k_{y}^{2}\right)+\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right)k_{x}k_{y};$\tabularnewline
 & $\left\{ R_{7},R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+\left[c_{2}\left(\Gamma_{1,0}+\Gamma_{1,3}\right)-c_{3}\left(\Gamma_{2,0}+\Gamma_{2,3}\right)\right]\left(k_{x}+k_{y}\right)+\left[c_{2}\left(\Gamma_{2,0}-\Gamma_{2,3}\right)-c_{3}\left(\Gamma_{1,0}-\Gamma_{1,3}\right)\right]\left(k_{x}-k_{y}\right)+\left[(1+i)\left(c_{2}+ic_{3}\right)\left(\Gamma_{2,+}k_{+}-\Gamma_{1,+}k_{-}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 137}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,2}k_{z}+\sum_{i=1}^{2}\left[c_{i,2}\Gamma_{i,0}k_{x}k_{y}+c_{4}\Gamma_{i,3}(k_{x}^{2}-k_{y}^{2})\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}-k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}+\Gamma_{1,2}+\Gamma_{2,1}-\Gamma_{2,2}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}-\Gamma_{1,2}+\Gamma_{2,1}+\Gamma_{2,2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right]$\tabularnewline
 & $\left\{ R_{2},R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,1}-\Gamma_{1,2}-\Gamma_{2,1}+\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,1}+\Gamma_{1,2}-\Gamma_{2,1}-\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 138}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $\{R_{15},R_{16}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{17},R_{18}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{20};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{3,1}k_{x}+c_{3}\Gamma_{0,2}k_{z}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{1},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}+\Gamma_{1,2}+\Gamma_{2,1}-\Gamma_{2,2}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{x}+\left(-\Gamma_{1,1}-\Gamma_{1,2}+\Gamma_{2,1}+\Gamma_{2,2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left[\left(\alpha_{1}\Gamma_{0,+}+\alpha_{2}\Gamma_{3,+}\right)k_{x}k_{y}+\alpha_{3}\Gamma_{1,+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right]$\tabularnewline
 & $\left\{ R_{2},R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left[\left(\Gamma_{1,1}-\Gamma_{1,2}-\Gamma_{2,1}+\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}-\Gamma_{1,3}-\Gamma_{2,0}-\Gamma_{2,3}\right)k_{y}\right]+c_{3}\left[\left(\Gamma_{1,1}+\Gamma_{1,2}-\Gamma_{2,1}-\Gamma_{2,2}\right)k_{x}+\left(\Gamma_{1,0}+\Gamma_{1,3}-\Gamma_{2,0}+\Gamma_{2,3}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{y}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 139}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}k_{x}k_{y}+c_{5}k_{z})\sigma_{1}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sigma_{1}\left(c_{5}k_{x}+c_{6}k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 140}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{C_{2x}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG141.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 141}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|0\frac{1}{2}0\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}(k_{x}+k_{y});$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}(k_{x}+k_{y});$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{2}k_{x}+\sigma_{1}k_{y});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{2}k_{x}+\sigma_{1}k_{y});$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{10};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}(k_{x}-k_{y})+c_{4}\sigma_{3}(k_{x}+k_{y});$ \tabularnewline




\multirow{1}{*}{$U$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{3}\sigma_{3}(k_{x}-k_{y})+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}-k_{y})\right]\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{9}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sigma_{1}\left(c_{5}k_{x}+c_{6}k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 142}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{1}{2}00\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}(c_{2}k_{z}+c_{3}k_{x});$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & \multirow{1}{*}{$\{R_{13},R_{14}\};$ } & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,2}k_{x}+\Gamma_{0,1}k_{y}\right)+c_{3}\left(\Gamma_{2,0}k_{x}-\Gamma_{1,3}k_{y}\right)$ \tabularnewline
 &  & $+c_{4}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,3}k_{y}\right)+k_{z}\left(c_{4}\Gamma_{1,1}-c_{6}\Gamma_{2,1}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{10};$  & $h_{0}^{\prime}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}(k_{x}^{2}-k_{y}^{2});$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{3}(k_{x}-k_{y});$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}+k_{y})\right]\sigma_{0}+c_{3}\sigma_{3}(k_{x}-k_{y})+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}-k_{y})\right]\sigma_{0}+c_{3}\sigma_{1}(k_{x}+k_{y})+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{3}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{2}k_{y}-A_{1}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{1}k_{y}-A_{2}k_{x}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{9}\right\} ,\left\{ R_{10}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 143}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 144}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{1}{3}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 145}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{2}{3}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 146}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{C_{3}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 147}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{+}+\alpha_{2}k_{-}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{+}+\alpha_{2}k_{-}^{2})+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 148}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{S_{6}^{+}|000\},\mathcal{T}$; Centrosymmetric;
without SOC}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{+}+\alpha_{2}k_{-}^{2})+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{-}+\alpha_{2}k_{+}^{2})+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[\sigma_{+}(\alpha_{1}k_{z}k_{+}+\alpha_{2}k_{-}^{2})+h.c.\right];$ \tabularnewline



\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{-}+h.c.\right]$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 149}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 150}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}-\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG151.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 151}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{1}{3}\},\{C_{21}^{\prime}|00\frac{2}{3}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}[b]{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 152}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{1}{3}\},\{C_{21}^{\prime\prime}|00\frac{2}{3}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}[b]{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}-\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$T'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$S'$;} & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 153}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{2}{3}\},\{C_{21}^{\prime}|00\frac{1}{3}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline












\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 154}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|00\frac{2}{3}\},\{C_{21}^{\prime\prime}|00\frac{1}{3}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y})+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}-\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)k_{y}\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\sum_{i=1}^{2}\sigma_{i}\left[c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{i,2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$T'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$S'$;} & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 155}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right]+c_{6}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right)\right];$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(k_{x}+\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+c_{3}k_{z}\right]+\sigma_{2}\left[c_{4}\left(\frac{k_{y}}{\sqrt{3}}-k_{x}\right)-c_{5}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sum_{i=0,3}\sigma_{i}c_{i,2}\left(k_{x}-\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{3}k_{z}\right]+\sigma_{2}\left[c_{4}\left(3k_{x}+\sqrt{3}k_{y}\right)+3c_{5}k_{z}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 156}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{\sigma_{v1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right];$ \tabularnewline



\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{3}k_{x}-\sigma_{1}k_{y});$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left[2A_{4}c_{3}+\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}-2A_{1}c_{6}\right]k_{x}+2\left(A_{6}c_{3}-A_{7}c_{4}-A_{2}c_{6}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left[2A_{6}c_{3}+\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}-2A_{2}c_{6}\right]k_{x}-2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 157}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{\sigma_{d1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multirow{1}{*}{$S'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 158}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{\sigma_{v1}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}(2c_{4}k_{x}-c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{x}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,3}k_{x}+\Gamma_{0,1}k_{y}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+\sigma_{3}(c_{2}k_{x}+c_{3}k_{z});$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}k_{z}\sigma_{i};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}k_{z}\sigma_{i};$ \tabularnewline
 & $\{R_{3},R_{3}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}k_{z}\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{3}k_{x}-\sigma_{1}k_{y});$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+\sqrt{3}c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}(k_{x}-\sqrt{3}k_{y})+c_{i,2}k_{z}\right]\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left[2A_{4}c_{3}+\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}-2A_{1}c_{6}\right]k_{x}+2\left(A_{6}c_{3}-A_{7}c_{4}-A_{2}c_{6}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left[2A_{6}c_{3}+\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}-2A_{2}c_{6}\right]k_{x}-2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{6}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{6}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 159}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{\sigma_{d1}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}-\Gamma_{0,3}k_{y}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+\sigma_{3}(c_{2}k_{y}+c_{3}k_{z});$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{6};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}-\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline





\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$T'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multirow{1}{*}{$S'$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 160}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{C_{3}^{+}|000\},\{\sigma_{d1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline



\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG161.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 161}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{C_{3}^{+}|000\},\{\sigma_{d1}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}(2c_{4}k_{y}+c_{5}k_{z})+\sigma_{3}\left[c_{4}(k_{x}^{2}-k_{y}^{2})+c_{5}k_{y}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}-\Gamma_{0,3}k_{y}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+\left[c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{3}k_{z}\right]\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}(\sigma_{1}k_{x}+\sigma_{3}k_{y});$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+\sqrt{3}c_{2}k_{x}-c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}(\sqrt{3}k_{x}+k_{y})+c_{i,2}k_{z}\right]\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 162}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+c_{2}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+c_{2}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 163}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime}|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,2}k_{x}+\Gamma_{3,1}k_{y}\right)+k_{z}\left(c_{4}\Gamma_{1,2}+c_{3}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{6};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline





\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{3}k_{x})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+c_{2}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left[c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{i,2}k_{z}\right]+c_{2}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 164}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime\prime}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}-c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}-c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\left(\sigma_{3}k_{x}-\sigma_{1}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+\sigma_{1}\left(c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{2}\left(c_{2}k_{y}-c_{3}k_{x}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(\left(c_{3}+c_{4}\right)k_{z}+c_{1}\right)+\sigma_{3}\left(\left(c_{3}-c_{4}\right)k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z}-2\left(A_{7}c_{3}+A_{2}c_{5}\right)k_{y}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{3}-2A_{1}c_{5}\right]k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{4}+c_{5}k_{z}\right)-2\left(A_{7}c_{3}-A_{1}c_{6}\right)k_{y}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{3}-2A_{2}c_{6}\right]k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sum_{i=0,3}\sigma_{i}\left[c_{i,1}+c_{i,2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{1}\left[c_{1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sum_{i=0,3}\sigma_{i}\left[c_{i,1}+c_{i,2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{1}\left[c_{1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{y}+\sigma_{1}\left(c_{2}k_{x}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{y}+\sigma_{1}\left(c_{2}k_{x}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 165}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime\prime}|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{y}\left(2c_{4}k_{x}-c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{x}k_{z}\right]$; \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,1}k_{x}-\Gamma_{0,2}k_{y}\right)+k_{z}\left(c_{4}\Gamma_{1,2}+c_{3}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\left(\Gamma_{i,1}k_{x}-\Gamma_{i,3}k_{y}\right)+c_{i,2}k_{z}\Gamma_{i,2}\right];$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{3}k_{x}-\sigma_{1}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+\sigma_{1}\left(c_{3}k_{x}+c_{4}k_{y}\right)-\sigma_{2}\left(c_{4}k_{x}-c_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sqrt{3}c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}(k_{x}-\sqrt{3}k_{y})+c_{i,2}k_{z}\right]\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline


\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(\left(c_{3}+c_{4}\right)k_{z}+c_{1}\right)+\sigma_{3}\left(\left(c_{3}-c_{4}\right)k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z}-2\left(A_{7}c_{3}+A_{2}c_{5}\right)k_{y}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{3}-2A_{1}c_{5}\right]k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{4}+c_{5}k_{z}\right)-2\left(A_{7}c_{3}-A_{1}c_{6}\right)k_{y}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{3}-2A_{2}c_{6}\right]k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sum_{i=0,3}\sigma_{i}\left[c_{i,1}+c_{i,2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{1}\left[c_{1}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{2}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{y}+\sigma_{1}\left(c_{2}k_{x}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right)+c_{2}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 166}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline



\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(k_{x}+\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(\sqrt{3}k_{x}-k_{y}\right)+c_{3}k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(k_{x}-\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{3}k_{z}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 167}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{rh}$; $\{S_{6}^{+}|000\},\{C_{21}^{\prime}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{y}^{2}-k_{x}^{2}\right)-c_{5}k_{y}k_{z}\right]$; \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sigma_{1}k_{x}\left(2c_{4}k_{y}+c_{5}k_{z}\right)+\sigma_{3}\left[c_{4}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{5}k_{y}k_{z}\right]$; \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,2}k_{x}+\Gamma_{3,1}k_{y}\right)+k_{z}\left(c_{4}\Gamma_{1,2}+c_{3}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left[c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{3}k_{z}\right];$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x}-c_{2}\sqrt{3}k_{y})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}(\sqrt{3}k_{x}+k_{y})+c_{i,2}k_{z}\right]\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+\sigma_{1}\left(c_{2}k_{y}+c_{3}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(k_{x}+\sqrt{3}k_{y}\right)+\sigma_{1}\left[c_{2}\left(\sqrt{3}k_{x}-k_{y}\right)+c_{3}k_{z}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 168}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 169}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{6}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{2},R_{12}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 170}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{5}{6}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{2},R_{12}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG171.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 171}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{3}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 172}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{2}{3}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 173}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{2}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{2},R_{12}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}+c_{6}\sigma_{3}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(\alpha_{1}k_{+}^{3}+\alpha_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{1}k_{x}+c_{2}k_{y}\right)+\sigma_{2}\left(c_{3}k_{x}+c_{4}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 174}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline



\multirow{1}{*}{$\Delta$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $\left[\sqrt{3}A_{1}\left(c_{3}-2c_{4}\right)+\sqrt{3}A_{2}\left(c_{4}-2c_{3}\right)+3\left(A_{4}c_{3}+A_{6}c_{4}\right)\right]k_{x}+3\left(A_{1}c_{3}-A_{2}c_{4}\right)k_{y}+\sqrt{3}\left[\left(2A_{4}+A_{6}\right)c_{4}-\left(A_{4}+2A_{6}\right)c_{3}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{+}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}k_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 175}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{2}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{11},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{11},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$K$;}&  $\{R_{2},R_{6}\};$  & $c_{3}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{2}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{6}\};$  & $c_{3}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{2}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+\sigma_{1}\left(c_{3}k_{x}+c_{4}k_{y}\right)-\sigma_{2}\left(c_{4}k_{x}-c_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{5}+c_{6}k_{z}\right)+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{6}k_{z}+c_{10}k^{2}+c_{11}k_{z}^{2}\right)+2\left[2\left(A_{1}-A_{2}\right)c_{5}+2A_{3}c_{7}+\left(A_{4}+A_{6}\right)c_{8}+A_{7}c_{9}\right]k_{x}k_{y}+\left[2\left(A_{4}+A_{6}\right)c_{5}+2A_{7}c_{7}+\left(A_{2}-A_{1}\right)c_{8}-A_{3}c_{9}\right]\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+A_{8}\left(c_{7}k_{z}+c_{10}k^{2}+c_{11}k_{z}^{2}\right)+2\left[-2A_{1}c_{5}+2\left(A_{2}-A_{3}\right)c_{6}+A_{4}c_{8}+\left(A_{6}+A_{7}\right)c_{9}\right]k_{x}k_{y}+\left[2A_{4}c_{5}+2\left(A_{6}+A_{7}\right)c_{6}+A_{1}c_{8}+\left(A_{3}-A_{2}\right)c_{9}\right]\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{3},R_{5}\right\} ;$  & $\Gamma_{1,0}\left(c_{3}k_{x}+c_{4}k_{y}\right)+\Gamma_{2,3}\left(c_{3}k_{y}-c_{4}k_{x}\right)+\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+\Gamma_{3,0}\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3},R_{5}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}\left(c_{5}+c_{6}k_{z}\right)+\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{5}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 176}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{2}|00\frac{1}{2}\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{11},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{13},R_{15}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,3}k_{z}+\left(\alpha_{1}\Gamma_{+,1}k_{-}^{2}+\alpha_{2}k_{z}\Gamma_{+,0}k_{+}+h.c.\right)$; \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $\{R_{2},R_{6}\};$  & $c_{3}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)+c_{2}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $c_{3}\left(\sigma_{1}k_{y}-\sigma_{2}k_{x}\right)+c_{2}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right)+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}k_{z}+h.c.\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}k_{z}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{2},R_{6}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{+}^{2}+h.c.\right);$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\left(\alpha_{1}\sigma_{+}k_{-}^{2}+h.c.\right);$ \tabularnewline

\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+\sigma_{1}\left(c_{3}k_{x}+c_{4}k_{y}\right)-\sigma_{2}\left(c_{4}k_{x}-c_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{5}+c_{6}k_{z}\right)+\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{6}k_{z}+c_{10}k^{2}+c_{11}k_{z}^{2}\right)+2\left[2\left(A_{1}-A_{2}\right)c_{5}+2A_{3}c_{7}+\left(A_{4}+A_{6}\right)c_{8}+A_{7}c_{9}\right]k_{x}k_{y}+\left[2\left(A_{4}+A_{6}\right)c_{5}+2A_{7}c_{7}+\left(A_{2}-A_{1}\right)c_{8}-A_{3}c_{9}\right]\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+A_{8}\left(c_{7}k_{z}+c_{10}k^{2}+c_{11}k_{z}^{2}\right)+2\left[-2A_{1}c_{5}+2\left(A_{2}-A_{3}\right)c_{6}+A_{4}c_{8}+\left(A_{6}+A_{7}\right)c_{9}\right]k_{x}k_{y}+\left[2A_{4}c_{5}+2\left(A_{6}+A_{7}\right)c_{6}+A_{1}c_{8}+\left(A_{3}-A_{2}\right)c_{9}\right]\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{3},R_{5}\right\} ;$  & $\Gamma_{1,0}\left(c_{3}k_{x}+c_{4}k_{y}\right)+\Gamma_{2,3}\left(c_{3}k_{y}-c_{4}k_{x}\right)+\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+\Gamma_{3,0}\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3},R_{5}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}\left(c_{5}+c_{6}k_{z}\right)+\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{5}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{7}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{3}+A_{7}c_{4}+\left(A_{2}-A_{1}\right)c_{5}-A_{3}c_{6}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+A_{3}c_{4}+\left(A_{4}+A_{6}\right)c_{5}+A_{7}c_{6}\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right)+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 177}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 178}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{6}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{2},R_{8}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{2},R_{4}\};$  & $\sigma_{0}\left(c_{2}k_{y}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 179}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{5}{6}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{2},R_{8}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{2},R_{4}\};$  & $\sigma_{0}\left(c_{2}k_{y}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 180}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{3}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG181.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 181}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{2}{3}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 182}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{2}\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right)+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{2},R_{8}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$S'$;} & $\{R_{2},R_{4}\};$  & $\sigma_{0}\left(c_{2}k_{y}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z})+c_{2}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1+i\sqrt{3}\right)c_{2}\sigma_{+}k_{+}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\left(1+c_{i,4}k^{2}+c_{i,5}k_{z}^{2}\right)\right]+\left[\left(c_{2}k_{+}^{3}+c_{2}k_{-}^{3}\right)\sigma_{+}+h.c.\right];$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}\left[c_{i,1}k^{2}+c_{i,2}k_{z}^{2}+c_{i,3}k_{z}\right]+\left[\left(1-i\sqrt{3}\right)c_{2}\sigma_{+}k_{-}^{2}+h.c.\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}k_{x}+c_{3}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\left[\left(3\sigma_{1}+\sqrt{3}\sigma_{2}\right)k_{x}+\left(\sqrt{3}\sigma_{1}-3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{0}c_{i,1}k_{z}+c_{2}\sigma_{1}\left(k_{x}+\frac{k_{y}}{\sqrt{3}}\right)+c_{2}\sigma_{2}\left(k_{y}-\frac{k_{x}}{\sqrt{3}}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{2}\sigma_{2}\left(\sqrt{3}k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 183}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|000\},\{\sigma_{v1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{6}\left(A_{4}k_{x}+A_{6}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{6}c_{5}-A_{2}c_{6}\right)k_{x}+\left(A_{1}c_{6}-A_{4}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{4}c_{5}-A_{1}c_{6}\right)k_{x}+\left(A_{2}c_{6}-A_{6}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{6}\left(A_{6}k_{x}+A_{4}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,2}k_{y}-\Gamma_{2,0}k_{x}\right)+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 184}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|000\},\{\sigma_{v1}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,3}\left(k_{x}^{2}-k_{y}^{2}\right)-2c_{i,2}\Gamma_{i,1}k_{x}k_{y}\right];$ \tabularnewline
 & $\{R_{9},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{12},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\Gamma_{i,3}\left(k_{x}^{2}-k_{y}^{2}\right)-2c_{i,2}\Gamma_{i,1}k_{x}k_{y}\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\sum_{i=1}^{3}\left[c_{i,1}\Gamma_{i,0}k_{z}+c_{i,2}\left(\Gamma_{i,1}k_{x}-\Gamma_{i,3}k_{y}\right)\right];$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right)+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$S'$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+\left(c_{2}\sigma_{1}+c_{4}\sigma_{2}\right)k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{2}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{6}\left(A_{4}k_{x}+A_{6}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{6}c_{5}-A_{2}c_{6}\right)k_{x}+\left(A_{1}c_{6}-A_{4}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{4}c_{5}-A_{1}c_{6}\right)k_{x}+\left(A_{2}c_{6}-A_{6}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{6}\left(A_{6}k_{x}+A_{4}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,2}k_{y}-\Gamma_{2,0}k_{x}\right)+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 185}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{2}\},\{\sigma_{v1}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{5},R_{11}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,0}k_{z}+c_{5}\left[2\Gamma_{0,1}k_{x}k_{y}+\Gamma_{0,3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+\left[\alpha_{1}k_{z}\left(k_{x}\Gamma_{+,1}+k_{y}\Gamma_{+,3}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $c_{1}\sigma_{0}+\left(c_{3}\sigma_{1}-c_{4}\sigma_{2}+c_{2}\sigma_{3}\right)k_{z};$ \tabularnewline
 & $\{R_{3},R_{3}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}+\Gamma_{0,3}k_{y}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{6}\left(A_{4}k_{x}+A_{6}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{6}c_{5}-A_{2}c_{6}\right)k_{x}+\left(A_{1}c_{6}-A_{4}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{4}c_{5}-A_{1}c_{6}\right)k_{x}+\left(A_{2}c_{6}-A_{6}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{6}\left(A_{6}k_{x}+A_{4}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,2}k_{y}-\Gamma_{2,0}k_{x}\right)+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+\left[\left(\alpha_{1}\Gamma_{1,+}+c_{2}\Gamma_{1,3}+c_{3}\Gamma_{2,0}\right)\left(k_{x}-\sqrt{3}k_{y}\right)+\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}+c_{4}\Gamma_{0,3}+c_{5}\Gamma_{3,3}\right)k_{z}+h.c.\right];$\tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{y}+\left[\left(\alpha_{1}\Gamma_{2,+}+c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)k_{x}+\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}+c_{4}\Gamma_{0,3}+c_{5}\Gamma_{3,3}\right)k_{z}+h.c.\right];$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 186}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{6}^{+}|00\frac{1}{2}\},\{\sigma_{v1}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{4},R_{10}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{5},R_{11}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{12}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{3,0}k_{z}+c_{5}\left[2\Gamma_{0,1}k_{x}k_{y}+\Gamma_{0,3}\left(k_{x}^{2}-k_{y}^{2}\right)\right]+\left[\alpha_{1}k_{z}\left(k_{x}\Gamma_{+,3}-k_{y}\Gamma_{+,1}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{3};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}k_{z}-\sigma_{3}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{6}\left(A_{4}k_{x}+A_{6}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{6}c_{5}-A_{2}c_{6}\right)k_{x}+\left(A_{1}c_{6}-A_{4}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(A_{4}c_{5}-A_{1}c_{6}\right)k_{x}+\left(A_{2}c_{6}-A_{6}c_{5}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{6}\left(A_{6}k_{x}+A_{4}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,2}k_{y}-\Gamma_{2,0}k_{x}\right)+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}+c_{i,2}k_{x}\right)+\left[k_{y}\left(\alpha_{1}\Gamma_{1,+}+c_{1}\Gamma_{1,3}+c_{2}\Gamma_{2,0}\right)+k_{z}\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}+c_{3}\Gamma_{0,3}+c_{4}\Gamma_{3,3}\right)+h.c.\right];$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 187}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline



\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{3}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(\frac{k_{x}}{\sqrt{3}}+k_{y}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sqrt{3}\sigma_{2}-3\sigma_{1}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(\frac{k_{x}}{\sqrt{3}}+k_{y}\right)\right];$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 188}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\{C_{21}^{\prime}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\left(\Gamma_{0,1}k_{x}-\Gamma_{3,2}k_{y}\right)k_{z}+\left[2\alpha_{1}k_{x}k_{y}\Gamma_{+,0}+i\alpha_{1}\Gamma_{+,3}\left(k_{x}^{2}-k_{y}^{2}\right)+\alpha_{2}k_{z}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{5}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{3},R_{6}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{3}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(\frac{k_{x}}{\sqrt{3}}+k_{y}\right)\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\left(\sqrt{3}\sigma_{2}-3\sigma_{1}\right)k_{x}+\left(\sqrt{3}\sigma_{1}+3\sigma_{2}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left[\sigma_{1}\left(k_{x}-\frac{k_{y}}{\sqrt{3}}\right)+\sigma_{2}\left(\frac{k_{x}}{\sqrt{3}}+k_{y}\right)\right];$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 189}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\{C_{21}^{\prime\prime}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 190}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{S_{3}^{+}|000\},\{C_{21}^{\prime\prime}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\left(\Gamma_{0,1}k_{y}+\Gamma_{3,2}k_{x}\right)k_{z}+\left[2\alpha_{1}k_{x}k_{y}\Gamma_{+,0}+i\alpha_{1}\Gamma_{+,3}\left(k_{x}^{2}-k_{y}^{2}\right)+\alpha_{2}k_{z}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{7};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left(\sigma_{2}k_{x}+\sigma_{1}k_{y}\right)k_{z};$ \tabularnewline
 & $R_{8};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left(\sigma_{2}k_{x}-\sigma_{1}k_{y}\right)k_{z};$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{3};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{3}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$S'$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{6}c_{3}+A_{7}c_{4}-A_{2}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{1}c_{6}-A_{4}c_{3}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+2\left(A_{4}c_{3}+A_{7}c_{4}-A_{1}c_{6}\right)k_{x}+\left[\left(\sqrt{3}A_{8}-A_{5}\right)c_{4}+2\left(A_{6}c_{3}-A_{2}c_{6}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+\left(c_{5}\sigma_{1}-c_{6}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG191.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 191}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\{C_{2}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+k_{z}\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Sp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 192}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|00\frac{1}{2}\},\{C_{2}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\left[2\alpha_{1}k_{x}k_{y}\Gamma_{+,0}+i\alpha_{1}\Gamma_{+,3}\left(k_{x}^{2}-k_{y}^{2}\right)+\alpha_{2}k_{z}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
 & $\{R_{16},R_{17}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+\left[2\alpha_{1}k_{x}k_{y}\Gamma_{+,0}+i\alpha_{1}\Gamma_{+,3}\left(k_{x}^{2}-k_{y}^{2}\right)+\alpha_{2}k_{z}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
 & $R_{18};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+\left[\alpha_{1}\left(k_{x}\Gamma_{+,3}+ik_{y}\Gamma_{+,0}\right)+\alpha_{2}k_{z}\Gamma_{+,1}+h.c.\right];$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{3}\left(k_{x}-\sqrt{3}k_{y}\right)+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+k_{z}\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 193}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|000\},\{C_{2}|00\frac{1}{2}\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{15};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,3}k_{z}+c_{5}k_{z}\left(\Gamma_{3,2}k_{x}+\Gamma_{0,1}k_{y}\right)+\left[c_{4}\Gamma_{+,0}\left(k_{x}^{2}-k_{y}^{2}\right)-2ic_{4}k_{x}k_{y}\Gamma_{+,3}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}+\Gamma_{0,3}k_{y}\right)+k_{z}\left(c_{3}\Gamma_{1,0}+c_{4}\Gamma_{2,0}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+c_{2}k_{y}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+k_{z}\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}\left(\sqrt{3}k_{x}+k_{y}\right)+\left[\alpha_{1}\Gamma_{1,+}\left(k_{x}-\sqrt{3}k_{y}\right)+\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}\right)k_{z}+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$Sp$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $\sum_{i=0,3}\Gamma_{i,0}\left(c_{i,1}+c_{i,2}k_{y}\right)+\left[\alpha_{1}k_{x}\Gamma_{1,+}+k_{z}\left(\alpha_{2}\Gamma_{0,+}+\alpha_{3}\Gamma_{3,+}\right)+h.c.\right];$\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 194}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{h}$; $\{C_{3}^{+}|000\},\{C_{21}^{\prime}|00\frac{1}{2}\},\{C_{2}|00\frac{1}{2}\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{12};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $R_{15};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\Gamma_{0,0}+c_{4}\Gamma_{0,3}k_{z}+c_{5}k_{z}\left(\Gamma_{0,1}k_{x}-\Gamma_{3,2}k_{y}\right)+\left[c_{6}\Gamma_{+,0}\left(k_{x}^{2}-k_{y}^{2}\right)-2ic_{6}k_{x}k_{y}\Gamma_{+,3}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$L$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$K$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline
 & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\left(\sigma_{1}k_{x}-\sigma_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{7};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(ic_{4}k_{+}k_{z}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $R_{8};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left(ic_{4}k_{-}k_{z}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}-\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{6};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\left[2\sigma_{1}k_{x}k_{y}+\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)\right];$ \tabularnewline

\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\left(\sigma_{1}k_{x}+\sigma_{3}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$Sp$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+k_{z}\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{2}c_{5}\right)k_{x}+\left[c_{5}A_{1}-c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left(2A_{7}c_{4}-A_{1}c_{5}\right)k_{x}-\left[c_{5}A_{2}+c_{4}\left(A_{5}-\sqrt{3}A_{8}\right)\right]k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-\sqrt{3}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(\sqrt{3}k_{x}+k_{y}\right)\right]+\sigma_{3}c_{3}\left(\sqrt{3}k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Tp$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{z}\left(c_{4}\Gamma_{0,1}+c_{5}\Gamma_{0,2}+c_{6}\Gamma_{3,1}+c_{7}\Gamma_{3,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 195}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline


\multirow{1}{*}{$R$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x}+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 196}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline

\multirow{1}{*}{$L$;}&  $\{R_{2},R_{3}\};$  & $\left[c_{1}+c_{2}(q_{x}^{2}+q_{y}^{2})+c_{3}q_{z}^{2}\right]\sigma_{0}+c_{4}q_{z}\sigma_{3}+\left[\sigma_{+}\left(\alpha_{1}q_{+}^{2}+\alpha_{2}q_{z}q_{-}\right)+h.c\right];$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 197}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right)+c_{3}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{-}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 198}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{+}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\sigma_{1}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]+\sigma_{2}\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i,1}k_{i}^{2}\right)\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{x}k_{y}+h.c.\right];$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i,1}k_{i}^{2}\right)\sigma_{0}+\left[\alpha_{1}\sigma_{+}k_{x}k_{y}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{4},R_{4}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,1}k_{x}-\Gamma_{0,2}k_{y}-\Gamma_{0,3}k_{z}\right);$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,1}k_{x}-\Gamma_{0,2}k_{y}-\Gamma_{3,3}k_{z}\right);$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{3}k_{z}+c_{1}\right)+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $\sigma_{0}\left(c_{2}k_{x}+c_{1}\right)+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{2}\};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i,1}k_{i}^{2}\right)+c_{3}\sigma_{3}k_{x}k_{y}+\left[\alpha_{1}\sigma_{+}k_{x}k_{y}+h.c.\right];$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i,1}k_{i}^{2}\right)+c_{3}\sigma_{3}k_{x}k_{y}+\left[\alpha_{1}\sigma_{+}k_{x}k_{y}+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{z}+c_{2}\Gamma_{2,0}k_{x}+c_{3}\Gamma_{1,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,2}\Gamma_{1,i}k_{x}+c_{i,3}\Gamma_{2,i}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 199}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{+}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\left[c_{3}k_{x}^{2}+c_{4}k_{y}^{2}-\left(c_{3}+c_{4}\right)k_{z}^{2}\right]\sigma_{1}+\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}-2k_{y}^{2}+k_{z}^{2}\right)\right]\sigma_{2}+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{5},R_{6}\};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+\sqrt{3}\left[c_{3}(k_{x}^{2}-k_{y}^{2})+c_{4}(k_{z}^{2}-k_{y}^{2})\right]\sigma_{1}+\left[c_{4}\left(-2k_{x}^{2}+k_{y}^{2}+k_{z}^{2}\right)-c_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]\sigma_{2}+c_{5}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{8};$  & $A_{0}c_{1}+c_{2}\left(A_{3}k_{x}+A_{1}k_{y}-A_{2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}q_{z}\sigma_{3}+c_{2}\left(q_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}q_{z}\sigma_{3}+c_{2}\left(q_{-}\sigma_{+}+h.c.\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}q_{z}\sigma_{3}+c_{2}\left(q_{-}\sigma_{+}+h.c.\right);$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}q_{z}+\left(\alpha_{1}\sigma_{+}q_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}p_{z}+\left(\alpha_{1}\sigma_{+}p_{-}+h.c.\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 200}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline


\multirow{1}{*}{$R$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left(c_{4}q_{x}-c_{5}q_{y}\right)\left(A_{4}+A_{6}\right)+\left(c_{4}q_{y}+c_{5}q_{x}\right)\left(A_{1}-A_{2}\right)+A_{7}\left(c_{6}q_{x}-c_{7}q_{y}\right)+A_{3}\left(c_{7}q_{x}+c_{6}q_{y}\right);$\tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{z}\right)+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG201.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 201}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline

\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{z}\right)+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 202}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline

\multirow{1}{*}{$L$;}&  $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2})\sigma_{0}+\left[(\alpha_{1}q_{+}^{2}+\alpha_{2}q_{z}q_{-})\sigma_{+}+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2})\sigma_{0}+\left[(\alpha_{1}q_{-}^{2}+\alpha_{2}q_{z}q_{+})\sigma_{+}+h.c.\right];$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{z}\right)+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 203}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{+}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$L$;}&  $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2})\sigma_{0}+\left[(\alpha_{1}q_{+}^{2}+\alpha_{2}q_{z}q_{-})\sigma_{+}+h.c.\right];$ \tabularnewline
 & $\{R_{3},R_{5}\};$  & $(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2})\sigma_{0}+\left[(\alpha_{1}q_{-}^{2}+\alpha_{2}q_{z}q_{+})\sigma_{+}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{9};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{z}\right)+c_{6}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 204}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{S_{61}^{+}|000\},\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}(q_{+}^{2}+2\sqrt{2}q_{-}q_{z})\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z});$ \tabularnewline



\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline


\multirow{1}{*}{$F$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}p_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}p_{-}+h.c.);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}-\left[c_{4}\left(A_{4}+A_{6}\right)+A_{7}c_{5}\right]\left(\sqrt{3}p_{x}+p_{y}\right)+\left[c_{4}\left(A_{1}-A_{2}\right)+A_{3}c_{5}\right]\left(p_{x}-\sqrt{3}p_{y}\right)+c_{6}\left[\left(A_{2}-A_{1}\right)p_{x}+\left(A_{4}+A_{6}\right)p_{y}\right]+c_{7}\left(A_{7}p_{y}-A_{3}p_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 205}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{+}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+k_{y}\left(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{4},R_{4}\};$  & $(c_{1}+c_{2}q^{2})\Gamma_{0,0}+\sum_{i}c_{1,i}\left\{ \Gamma_{i,3}\left(q_{x}^{2}+q_{y}^{2}-2q_{z}^{2}\right)-\left[\sqrt{2}e^{i\frac{7\pi}{12}}\Gamma_{i,+}\left(\sqrt{2}q_{+}q_{z}-q_{-}^{2}\right)+h.c.\right]\right\} ;$ \tabularnewline
 & $\{R_{5},R_{6}\};$  & $c_{1}\Gamma_{0,0};$ \tabularnewline
 & $\{R_{11},R_{11}\};$  & $(c_{1}+c_{2}q^{2})\Gamma_{0,0}+\sum_{i}c_{1,i}\left\{ \Gamma_{i,3}\left(q_{x}^{2}+q_{y}^{2}-2q_{z}^{2}\right)-\left[\sqrt{2}e^{i\frac{7\pi}{12}}\Gamma_{i,+}\left(\sqrt{2}q_{+}q_{z}-q_{-}^{2}\right)+h.c.\right]\right\} ;$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $c_{1}\Gamma_{0,0};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}+c_{3}k_{z}\right)\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{5}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\Gamma_{0,0}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{i,3}k_{x}+c_{i,2}\Gamma_{i,1}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}c_{5}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{0,1}-c_{3}\Gamma_{0,2}+c_{4}\Gamma_{3,1}+c_{5}\Gamma_{3,2}\right)+k_{z}\left(c_{6}\Gamma_{1,1}-c_{7}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 206}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{S_{61}^{+}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{6},R_{7}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{z}q_{-}+q_{+}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $c_{1}A_{0}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{z}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{x}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{y}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$H$;}&  $\{R_{5},R_{6}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{+}q_{z}+q_{-}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{8};$  & $A_{0}c_{1}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{y}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{x}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{z}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{6}k_{x}k_{y}+A_{4}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
 & $\{R_{13},R_{14}\};$  & $(c_{1}+c_{2}q^{2})\sigma_{0}+\left[\alpha_{1}\left(2\sqrt{2}q_{+}q_{z}+q_{-}^{2}\right)\sigma_{+}+h.c.\right];$ \tabularnewline
 & $R_{16};$  & $A_{0}c_{1}+\text{diag}\left[c_{2}k_{x}^{2}+c_{3}k_{y}^{2}+c_{4}k_{z}^{2},\ c_{2}k_{z}^{2}+c_{3}k_{x}^{2}+c_{4}k_{y}^{2},\ c_{2}k_{y}^{2}+c_{3}k_{z}^{2}+c_{4}k_{x}^{2}\right]+c_{5}(A_{6}k_{x}k_{y}+A_{4}k_{x}k_{z}+A_{7}k_{y}k_{z});$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{7},R_{7}\};$  & $c_{1}\Gamma_{0,0}+\sum_{i=1}^{3}c_{i,1}\left[\Gamma_{i,3}q_{z}+\left((-1)^{5/12}q_{-}\Gamma_{i,+}+h.c.\right)\right]$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{3}\};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}q_{-}+h.c.);$ \tabularnewline
\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+\sigma_{1}\left(c_{3}k_{x}+c_{4}k_{y}\right)+\sigma_{2}\left(c_{5}k_{x}+c_{6}k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$F$;} & $\{R_{2},R_{6}\};$  & $\left(c_{1}+c_{2}p_{z}\right)\sigma_{0}+(\alpha_{1}\sigma_{+}p_{+}+h.c.);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{$ $}\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{4}\left(A_{4}+A_{6}\right)+c_{5}\left(A_{1}-A_{2}\right)+A_{7}c_{6}+A_{3}c_{7}\right]q_{x}+\left[c_{4}\left(A_{1}-A_{2}c_{5}\right)-c_{5}\left(A_{4}+A_{6}\right)+A_{3}c_{6}-A_{7}c_{7}\right]q_{y};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+A_{8}c_{3}p_{z}+\left[\left(\sqrt{3}A_{4}+A_{1}\right)c_{5}+\left[\sqrt{3}\left(A_{6}+A_{7}\right)+A_{3}-A_{2}\right]c_{4}-A_{1}c_{6}+\left(A_{3}-A_{2}\right)c_{7}\right]p_{x}+\left[\left(A_{4}-\sqrt{3}A_{1}\right)c_{5}+\left[\sqrt{3}\left(A_{2}-A_{3}\right)+A_{6}+A_{7}\right]c_{4}+A_{4}c_{6}+\left(A_{6}+A_{7}\right)c_{7}\right]p_{y}$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 207}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,1}k_{y}\right)+c_{2}\sigma_{2}\left(k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+c_{2}\sigma_{2}\left(k_{z}-k_{x}\right)+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+c_{2}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left\{ \sigma_{+}\left[c_{2}\left(k_{x}^{2}-k_{y}^{2}\right)+ic_{3}k_{x}k_{y}\right]+h.c.\right\} ;$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left\{ \sigma_{+}\left[c_{2}\left(k_{x}^{2}-k_{y}^{2}\right)+ic_{3}k_{x}k_{y}\right]+h.c.\right\} ;$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 208}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,1}k_{y}\right)+c_{2}\sigma_{2}\left(k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+c_{2}\sigma_{2}\left(k_{z}-k_{x}\right)+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+c_{2}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left\{ \sigma_{+}\left[c_{2}\left(k_{x}^{2}-k_{y}^{2}\right)+ic_{3}k_{x}k_{y}\right]+h.c.\right\} ;$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}-\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{z}+c_{i,2}k^{2}+c_{i,3}k_{z}^{2}\right)+\left\{ \sigma_{+}\left[c_{2}\left(k_{x}^{2}-k_{y}^{2}\right)+ic_{3}k_{x}k_{y}\right]+h.c.\right\} ;$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\left(\sigma_{1}k_{x}+\sigma_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 209}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\sigma_{0}\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(q_{x}^{2}+q_{y}^{2})+c_{3}q_{z}^{2}\right]\sigma_{0}+\left[c_{4}(q_{x}^{2}-q_{y}^{2})-c_{5}q_{x}q_{z}\right]\sigma_{3}+\left[(2c_{4}q_{x}q_{y}+c_{5}q_{y}q_{z}+ic_{6}q_{z})\sigma_{+}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{x}^{2}\right)\sigma_{0}+c_{6}\sigma_{3}k_{y}k_{z}+\left[\sigma_{+}\left(\alpha_{1}k_{x}+\alpha_{2}(k_{y}^{2}-k_{z}^{2})\right)+h.c.\right];$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,1}k_{y}\right)+c_{2}\sigma_{2}\left(k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+c_{2}\sigma_{2}\left(k_{z}-k_{x}\right)+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+c_{2}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}-c_{i,1}k_{z}\right)+\sum_{i=1}^{2}\sigma_{1}\left[c_{i,2}k_{x}+c_{i,3}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 210}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{6}\sigma_{2}k_{y}$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{3};$  & $\left[c_{1}+c_{2}(q_{x}^{2}+q_{y}^{2})+c_{3}q_{z}^{2}\right]\sigma_{0}+\left[c_{4}(q_{x}^{2}-q_{y}^{2})-c_{5}q_{x}q_{z}\right]\sigma_{3}+\left[(2c_{4}q_{x}q_{y}+c_{5}q_{y}q_{z}+ic_{6}q_{z})\sigma_{+}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{x}+c_{3}\left[\sigma_{2}\left(k_{y}+k_{z}\right)+\sigma_{3}\left(k_{y}-k_{z}\right)\right];$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,1}k_{y}\right)+c_{2}\sigma_{2}\left(k_{y}-k_{x}\right)+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right)+c_{2}\sigma_{2}\left(k_{z}-k_{x}\right)+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}c_{i,1}k_{x}+c_{2}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}-c_{i,1}k_{z}\right)+\sum_{i=1}^{2}\sigma_{1}\left[c_{i,2}k_{x}+c_{i,3}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG21.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 21}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 22}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 23}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{C_{2y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 24}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline





\multicolumn{1}{l}{$W$;} & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{x};$\tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y}+c_{5}\sigma_{2}k_{z};$\tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{x}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 25}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{\sigma_{y}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$H$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 26}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline



\multicolumn{1}{l}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline

\multicolumn{1}{l}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline


\multicolumn{1}{l}{$P$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{1,i}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{1,i}\sigma_{i}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{1,i}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{1,i}\sigma_{i}k_{z};$ \tabularnewline


\multicolumn{1}{l}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$H$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 27}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multicolumn{1}{l}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{6}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 28}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}00\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline



\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
$\Delta$;& &\tabularnewline




\multicolumn{1}{l}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multicolumn{1}{l}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 29}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline

\multicolumn{1}{l}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,1}k_{x}+c_{3}\Gamma_{0,3}k_{y}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\{R_{5},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,1}k_{x}+c_{3}\Gamma_{0,3}k_{y}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline


\multicolumn{1}{l}{$P$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multicolumn{1}{l}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 30}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}00\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline

\multicolumn{1}{l}{$Y$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline

\multicolumn{1}{l}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG211.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 211}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{C_{2a}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right)+c_{3}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)p_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)p_{y}\right];$\tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sqrt{3}\sigma_{2}-\sigma_{1}\right)p_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)p_{y}\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)p_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)p_{y}\right];$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 212}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{C_{2a}|\frac{1}{4}\frac{3}{4}\frac{3}{4}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{4},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,2}q_{x}+\Gamma_{3,1}q_{y}-\Gamma_{3,3}q_{z}\right);$ \tabularnewline
 & $R_{8};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[\Gamma_{0,2}\left(k_{x}+k_{y}\right)+\Gamma_{3,3}\left(k_{x}-k_{y}\right)+\sqrt{2}\Gamma_{3,1}k_{z}\right];$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{4},R_{8}\};$  & $\left(c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{7}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}+c_{4}k_{z})\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}+c_{4}k_{z})\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{2}k_{x}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{2}k_{z}+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,0}k_{y}\right)+\left[k_{x}\left(\alpha\Gamma_{2,+}-c_{4}\Gamma_{2,3}\right)+k_{y}\left(\alpha\Gamma_{1,+}+c_{4}\Gamma_{1,3}\right)+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 213}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{C_{2a}|\frac{3}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{4},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{0,2}q_{x}+\Gamma_{3,1}q_{y}-\Gamma_{3,3}q_{z}\right);$ \tabularnewline
 & $R_{8};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[\Gamma_{0,2}\left(k_{x}+k_{y}\right)+\Gamma_{3,3}\left(k_{x}-k_{y}\right)+\sqrt{2}\Gamma_{3,1}k_{z}\right];$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{2},R_{6}\};$  & $\left(c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{7}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}+c_{4}k_{z})\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{2}k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}+c_{4}k_{z})\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{2}k_{x}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{2}k_{z}+c_{3}\left(\Gamma_{1,0}k_{x}+\Gamma_{2,0}k_{y}\right)+\left[k_{x}\left(\alpha\Gamma_{2,+}-c_{4}\Gamma_{2,3}\right)+k_{y}\left(\alpha\Gamma_{1,+}+c_{4}\Gamma_{1,3}\right)+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 214}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{-}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{C_{2a}|\frac{1}{2}00\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sqrt{3}(k_{x}^{2}-k_{y}^{2})\sigma_{1}+(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2})\sigma_{3}\right]+c_{4}k_{x}k_{y}k_{z}\sigma_{2}$ \tabularnewline
 & $R_{4};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}-A_{2}k_{y}+A_{1}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sqrt{3}\sigma_{1}\left(k_{x}^{2}-k_{z}^{2}\right)+\sigma_{3}\left(k_{x}^{2}+k_{z}^{2}-2k_{y}^{2}\right)\right]+c_{4}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $R_{9};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}+A_{1}k_{y}+A_{2}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $A_{0}c_{1}-c_{2}\left(A_{3}k_{x}+A_{1}k_{y}+A_{2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\left\{ q_{z}\sigma_{3}-\left[(-1)^{7/12}q_{+}\sigma_{-}+h.c.\right]\right\} ;$ \tabularnewline
 & $R_{8};$  & $c_{1}\sigma_{0}+c_{2}\left\{ q_{z}\sigma_{3}-\left[(-1)^{7/12}q_{+}\sigma_{-}+h.c.\right]\right\} ;$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\left\{ q_{z}\sigma_{3}-\left[(-1)^{7/12}q_{+}\sigma_{-}+h.c.\right]\right\} ;$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z}+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{x}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}c_{1}+\sum_{i=0,3}\sigma_{i}\left(c_{i,1}k_{y}+c_{i,2}k^{2}+c_{i,3}k_{y}^{2}\right)+\left[\sigma_{+}\left(c_{2}k_{x}k_{z}+ic_{3}\left(k_{x}^{2}-k_{z}^{2}\right)\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{x}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}-\sigma_{2}\right)q_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z}+c_{4}\left[\left(\sigma_{1}-\sqrt{3}\sigma_{2}\right)q_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)q_{y}\right];$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)p_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)p_{y}\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sqrt{3}\sigma_{2}-\sigma_{1}\right)p_{x}+\left(\sqrt{3}\sigma_{1}+\sigma_{2}\right)p_{y}\right];$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z}+c_{5}\left[\left(\sigma_{1}+\sqrt{3}\sigma_{2}\right)p_{x}+\left(\sigma_{2}-\sqrt{3}\sigma_{1}\right)p_{y}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 215}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{2}q_{z})\sigma_{0}+c_{3}\left(\sigma_{1}q_{y}-\sigma_{3}q_{x}\right);$ \tabularnewline


\multirow{1}{*}{$T$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{2}\left(k_{z}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y}+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left[\left(A_{6}-A_{4}\right)c_{5}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{5}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+\left[\left(A_{4}+A_{6}\right)c_{5}+\left(A_{2}-A_{1}\right)c_{6}\right]k_{x}-\left[\left(A_{6}-A_{4}\right)c_{5}+\left(A_{1}+A_{2}\right)c_{6}\right]k_{y};$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 216}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{3}\left[c_{4}\left(q_{x}^{2}-q_{y}^{2}\right)-c_{5}q_{x}q_{z}\right]+\left[\sigma_{+}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{2}q_{z})\sigma_{0}+c_{3}\left(\sigma_{1}q_{y}-\sigma_{3}q_{x}\right);$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{2}\left(k_{z}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y}+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 217}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q^{2}\right)\sigma_{0}+c_{3}\left[2\sigma_{1}q_{y}\left(q_{x}-\sqrt{2}q_{z}\right)+\sigma_{3}\left(2\sqrt{2}q_{x}q_{z}+q_{x}^{2}-q_{y}^{2}\right)\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right);$ \tabularnewline


\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $(c_{1}+c_{2}q_{z})\sigma_{0}+c_{3}\left(\sigma_{1}q_{y}-\sigma_{3}q_{x}\right);$ \tabularnewline


\multirow{1}{*}{$F$;}&  $R_{3};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}+k_{z}\right)\right]\sigma_{0}+c_{3}\left[\sqrt{3}\sigma_{1}\left(k_{x}+k_{y}\right)+\sigma_{3}\left(k_{x}-k_{y}-2k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}+\left(A_{6}c_{4}-c_{7}A_{2}-2c_{5}A_{7}\right)\left(\sqrt{3}p_{x}-p_{y}\right)+\left[c_{6}A_{1}-A_{4}c_{4}+c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)\right]\left(p_{x}+\sqrt{3}p_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}+\left(A_{1}c_{6}-A_{4}c_{4}-2c_{5}A_{7}\right)\left(\sqrt{3}p_{x}-p_{y}\right)+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)-A_{6}c_{4}+A_{2}c_{6}\right]\left(p_{x}+\sqrt{3}p_{y}\right);$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 218}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $\{R_{5},R_{6}\};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+\left(c_{4}\sigma_{1}+c_{5}\sigma_{2}\right)\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right)+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\Gamma_{0,0}+c_{3}\left[\Gamma_{3,1}\left(k_{x}^{2}-k_{y}^{2}\right)-\frac{\Gamma_{3,2}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right]+\left\{ \alpha_{1}\left[\Gamma_{+,1}\left(k_{x}^{2}-k_{y}^{2}\right)-\frac{\Gamma_{+,2}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right]+h.c.\right\} ;$ \tabularnewline
 & $\{R_{9},R_{10}\};$  & $c_{1}S_{0,0}+c_{2}\left(S_{1,1}k_{x}+S_{1,2}k_{y}-S_{1,3}k_{z}\right)+c_{3}\left(S_{2,1}k_{x}+S_{2,2}k_{y}-S_{2,3}k_{z}\right)+c_{4}\left(S_{3,4}k_{x}-S_{3,6}k_{y}-S_{3,7}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+c_{3}(\sigma_{3}q_{x}-q_{y}\sigma_{1});$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]\sigma_{0}+c_{4}\sigma_{3}k_{y}+\left(c_{3}\sigma_{1}+c_{5}\sigma_{2}\right)\left(k_{x}-k_{z}\right);$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{y}^{2}\right)+h.c.\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y}+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{3}k_{z}+\left[\left(A_{6}-A_{7}\right)c_{4}-\left(A_{2}+A_{3}\right)c_{5}\right]k_{x}-\left[\left(A_{6}+A_{7}\right)c_{4}+\left(A_{3}-A_{2}\right)c_{5}\right]k_{y};$ \tabularnewline
 & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{3}k_{z}+\left[\left(A_{6}+A_{7}\right)c_{4}+\left(A_{3}-A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{7}\right)c_{4}-\left(A_{2}+A_{3}\right)c_{5}\right]k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 219}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{C_{31}^{-}|000\},\{C_{2z}|000\},\{C_{2x}|000\},\{\sigma_{da}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{3},R_{4}\};$  & $c_{2}\sigma_{3}q_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\sqrt{2}\Gamma_{0,3}q_{x}-\sqrt{2}\Gamma_{0,1}q_{y}+\Gamma_{3,0}q_{z}\right)+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}q_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{3}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}+c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}\left[\sigma_{3}q_{x}-q_{y}\left(\sigma_{-}+\sigma_{+}\right)\right];$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]\sigma_{0}+\sum_{i=1}^{3}\sigma_{i}\left[c_{i,1}k_{x}+c_{i,2}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{2}\left(k_{z}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y}+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 220}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{C_{31}^{-}|000\},\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\{\sigma_{da}|\frac{1}{2}00\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{3};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{y}^{2}-k_{x}^{2}\right)-\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{6}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\Gamma_{0,0}+c_{3}\left[\Gamma_{3,1}\left(k_{x}^{2}-k_{y}^{2}\right)-\frac{\Gamma_{3,2}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right]+\left\{ \alpha_{1}\left[\Gamma_{+,1}\left(k_{x}^{2}-k_{y}^{2}\right)-\frac{\Gamma_{+,2}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right]+h.c.\right\} ;$ \tabularnewline
 & $\{R_{9},R_{10}\};$  & $c_{1}S_{0,0}+c_{2}\left(S_{1,1}k_{x}+S_{1,2}k_{y}-S_{1,3}k_{z}\right)+c_{3}\left(S_{2,1}k_{x}+S_{2,2}k_{y}-S_{2,3}k_{z}\right)+c_{4}\left(S_{3,4}k_{x}-S_{3,6}k_{y}-S_{3,7}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{9};$  & $c_{1}\sigma_{0};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0};$ \tabularnewline
 & $R_{16};$  & $c_{1}\Gamma_{0,0}+\sqrt{6}\left(c_{2}-c_{3}\right)\left(\Gamma_{3,1}k_{y}+\Gamma_{3,2}k_{z}\right)+k_{x}\left[(3-i)c_{2}+4ic_{3}\right]\Gamma_{+,3}+\left(k_{y}\Gamma_{+,1}-k_{z}\Gamma_{+,2}\right)\left[\left(2ic_{2}+(3+i)c_{3}\right)\right];$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$\Delta$;}&  $\{R_{3},R_{4}\};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z}+\left[\alpha_{1}\sigma_{+}\left(k_{x}^{2}-k_{z}^{2}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}\left[\sigma_{3}q_{x}-q_{y}\left(\sigma_{-}+\sigma_{+}\right)\right];$ \tabularnewline
\multirow{1}{*}{$D$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{2}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{3}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)\left(k_{x}+k_{y}\right)+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;}&  $R_{6};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}+k_{y}\right)+\frac{c_{3}\sigma_{3}\left(-k_{x}+k_{y}+2k_{z}\right)}{\sqrt{3}};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}-\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{x}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+\left[\left(A_{4}+A_{6}\right)c_{4}+\left(A_{2}-A_{1}\right)c_{5}\right]k_{x}+\left[\left(A_{6}-A_{4}\right)c_{4}+\left(A_{1}+A_{2}\right)c_{5}\right]k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\sqrt{2}\left(A_{1}c_{6}-A_{4}c_{4}\right)\right]q_{x}+2\left[\sqrt{3}\left(A_{2}c_{6}-A_{6}c_{4}\right)+A_{7}c_{5}\right]q_{y};$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+\left[c_{5}\left(A_{5}-\sqrt{3}A_{8}\right)+2\left(A_{2}c_{6}-A_{6}c_{4}\right)\right]q_{x}+2\left(A_{4}c_{4}+A_{7}c_{5}-A_{1}c_{6}\right)q_{y};$\tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}+c_{5}\left[\left(p_{x}+\sqrt{3}p_{y}\right)\left(A_{5}-\sqrt{3}A_{8}\right)+2A_{7}\left(\sqrt{3}p_{x}-p_{y}\right)\right]+\left[\left(A_{4}+\sqrt{3}A_{6}\right)c_{4}-\left(A_{1}+\sqrt{3}A_{2}\right)c_{6}\right]p_{x}+\left[\left(\sqrt{3}A_{4}-A_{6}\right)c_{4}+\left(A_{2}-\sqrt{3}A_{1}\right)c_{6}\right]p_{y};$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}p_{z}+c_{5}\left[\left(p_{x}+\sqrt{3}p_{y}\right)\left(A_{5}-\sqrt{3}A_{8}\right)+2A_{7}\left(\sqrt{3}p_{x}-p_{y}\right)\right]+\left[\left(\sqrt{3}A_{4}-A_{6}\right)c_{4}+\left(A_{2}-\sqrt{3}A_{1}\right)c_{6}\right]p_{x}-\left[\left(A_{4}+\sqrt{3}A_{6}\right)c_{4}-\left(A_{1}+\sqrt{3}A_{2}\right)c_{6}\right]p_{y}$\tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG221.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 221}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|000\},\{\sigma_{z}|000\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline


\multirow{1}{*}{$T$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 222}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{-}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{z}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $\{R_{12},R_{13}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2})\Gamma_{0,0}+\left[\alpha_{1}\Gamma_{+,0}\left(k_{x}^{2}-k_{z}^{2}\right)+\alpha_{2}k_{x}k_{z}\Gamma_{+,3}+\alpha_{3}k_{y}\Gamma_{+,2}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\Gamma_{0,0}+\left(c_{3}\Gamma_{1,0}+c_{4}\Gamma_{2,0}\right)\left(2k_{x}^{2}-k_{y}^{2}-k_{z}^{2}\right)-\sqrt{3}\left(c_{3}\Gamma_{2,3}-c_{4}\Gamma_{1,3}\right)\left(k_{y}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{14};$  & $c_{1}S_{0,0}+c_{2}\left(k_{x}S_{1}^{\prime}+k_{y}S_{2}^{\prime}+k_{z}S_{3}^{\prime}\right)+c_{3}\left(k_{x}S_{4}^{\prime}+k_{y}S_{5}^{\prime}+k_{z}S_{6}^{\prime}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}\left(k_{x}-k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;}&  $R_{9};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+c_{6}\sigma_{2}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 &  & \tabularnewline
\multicolumn{3}{l}{Here, $S_{1}^{\prime}=3S_{0,1}-2S_{2,0}+2\sqrt{3}S_{2,8}-3S_{3,1}$,
$S_{2}^{\prime}=3\left(-S_{1,1}+S_{1,2}+S_{2,4}+S_{2,6}\right)$,
$S_{3}^{\prime}=3\left(S_{0,3}-S_{1,1}-S_{2,4}+S_{3,3}\right)$,}\tabularnewline
\multicolumn{3}{l}{$S_{4}^{\prime}=3\left(-S_{0,3}+S_{1,2}-S_{2,6}+S_{3,3}\right)$,
$S_{5}^{\prime}=-\left(3S_{1,3}+2S_{2,0}+3S_{2,5}+3S_{2,7}+\sqrt{3}S_{2,8}\right)$,
$S_{6}^{\prime}=\left(3S_{0,2}-2S_{2,0}+3S_{2,5}-\sqrt{3}S_{2,8}+3S_{3,2}\right)$.}\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right];$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right];$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right];$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 223}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|000\},\{\sigma_{z}|000\},\{C_{2c}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{12};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\sigma_{2}k_{x}k_{y}k_{z};$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left(c_{1}+c_{2}k^{2}\right)\Gamma_{0,0}+\left(c_{3}\Gamma_{1,0}+c_{4}\Gamma_{2,0}\right)\left(2k_{x}^{2}-k_{y}^{2}-k_{z}^{2}\right)-\sqrt{3}\left(c_{3}\Gamma_{2,3}-c_{4}\Gamma_{1,3}\right)\left(k_{y}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{14};$  & $c_{1}S_{0,0}+c_{2}\left(k_{x}S_{1}^{\prime}+k_{y}S_{2}^{\prime}+k_{z}S_{3}^{\prime}\right)+c_{3}\left(k_{x}S_{4}^{\prime}+k_{y}S_{5}^{\prime}+k_{z}S_{6}^{\prime}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}+c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}\left(k_{x}-k_{z}\right);$ \tabularnewline

\multirow{1}{*}{$T$;}&  $R_{10};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
 &  & \tabularnewline
\multicolumn{3}{l}{Definition of $S_{i}^{\prime}$, see SG 222. }\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{x}+A_{1}k_{y}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{2}k_{y}-A_{1}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{y}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{9}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left(A_{1}k_{x}+A_{2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 224}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}$; $\{S_{61}^{-}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{z}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2c}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{12};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline

\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;}&  $R_{10};$  & $\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+c_{6}\sigma_{2}\left(k_{x}^{2}-k_{y}^{2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$T$;} & $\left\{ R_{5}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right];$\tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right];$\tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(-A_{1}+A_{2}+A_{4}+A_{6}\right)k_{x}+\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{y}\right];$\tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{10}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{z}+c_{4}\left[\left(A_{1}-A_{2}-A_{4}-A_{6}\right)k_{y}-\left(A_{1}+A_{2}-A_{4}+A_{6}\right)k_{x}\right];$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 225}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|000\},\{\sigma_{z}|000\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{5};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{1}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)-\sigma_{3}\left(c_{4}q_{x}^{2}-c_{4}q_{y}^{2}-c_{5}q_{x}q_{z}\right);$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{1}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)+\sigma_{3}\left(c_{4}q_{x}^{2}-c_{4}q_{y}^{2}-c_{5}q_{x}q_{z}\right);$ \tabularnewline
\multirow{1}{*}{$W$;}&  $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]+\sigma_{3}c_{3}\left(k_{y}-k_{z}\right)+\sigma_{1}\left[c_{4}k_{x}+c_{5}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 226}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{-}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{z}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{z}+c_{5}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,1}q_{x}+\Gamma_{0,2}q_{y}\right)+q_{z}\left(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}q_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{13},R_{16}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\{R_{14},R_{15}\};$  & $c_{1}\sigma_{0}+\left(c_{2}\sigma_{1}-c_{3}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $R_{20};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline



\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{x}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{y}+k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$Z$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 227}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{-}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\{\sigma_{x}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\{\sigma_{z}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\{C_{2c}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{11};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{13};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{14};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
\multirow{1}{*}{$L$;}&  $R_{5};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{1}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)-\sigma_{3}\left(c_{4}q_{x}^{2}-c_{4}q_{y}^{2}-c_{5}q_{x}q_{z}\right);$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}q^{2}+c_{3}q_{z}^{2}\right)\sigma_{0}+\sigma_{1}q_{y}\left(2c_{4}q_{x}+c_{5}q_{z}\right)+\sigma_{3}\left(c_{4}q_{x}^{2}-c_{4}q_{y}^{2}-c_{5}q_{x}q_{z}\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\left[\left(\sigma_{1}-\sigma_{2}\right)k_{y}-\left(\sigma_{1}+\sigma_{2}\right)k_{z}\right];$ \tabularnewline
 & $R_{12};$  & $c_{1}\sigma_{0}+c_{2}\left[\left(\sigma_{1}+\sigma_{2}\right)k_{y}+\left(\sigma_{2}-\sigma_{1}\right)k_{z}\right];$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]+\sigma_{3}c_{3}\left(k_{y}-k_{z}\right)+\sigma_{1}\left[c_{4}k_{x}+c_{5}\left(k_{y}+k_{z}\right)\right];$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 228}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{f}$; $\{S_{61}^{-}|\frac{3}{4}\frac{3}{4}\frac{3}{4}\},\{\sigma_{x}|\frac{3}{4}\frac{3}{4}\frac{3}{4}\},\{\sigma_{z}|\frac{3}{4}\frac{3}{4}\frac{3}{4}\},\{C_{2c}|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{11};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{12};$  & $\left(c_{1}+c_{2}k^{2}+c_{3}k_{y}^{2}\right)\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{z};$ \tabularnewline
 & $R_{14};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$L$;} & $\{R_{7},R_{8}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left(\Gamma_{3,1}q_{x}+\Gamma_{0,2}q_{y}\right)+q_{z}\left(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2}\right);$ \tabularnewline
 & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}q_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{13},R_{14}\};$  & $c_{1}\Gamma_{0,0}+c_{3}\Gamma_{0,1}\left(k_{y}+k_{z}\right)-c_{3}\Gamma_{3,2}\left(k_{y}-k_{z}\right)+\left[\alpha_{1}k_{x}\Gamma_{+,1}-i\alpha_{2}\Gamma_{+,0}\left(k_{y}-k_{z}\right)+\alpha_{2}\Gamma_{+,3}\left(k_{y}+k_{z}\right)+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{x}\right)\sigma_{0}+c_{3}\sigma_{3}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{4},R_{8}\};$  & $\left[c_{1}+c_{2}\left(k_{y}-k_{z}\right)\right]\sigma_{0}+\left(c_{3}\sigma_{1}+c_{4}\sigma_{2}\right)k_{x}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)\left(k_{y}+k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{z}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{z}\right)+c_{5}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 229}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|000\},\{\sigma_{z}|000\},\{C_{2c}|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;}&  $R_{3};$  & $(c_{1}+c_{2}k^{2})\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{4};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right);$ \tabularnewline
 & $R_{5};$  & $c_{1}A_{0}+c_{2}\left(A_{7}k_{x}+A_{6}k_{y}+A_{4}k_{z}\right);$ \tabularnewline


\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline


\multirow{1}{*}{$F$;}&  $R_{3};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}+k_{y}\right)+\frac{c_{3}\sigma_{3}\left(k_{x}-k_{y}-2k_{z}\right)}{\sqrt{3}};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]+\sigma_{3}c_{3}\left(k_{x}-k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{3}+c_{4}p_{z}\right)+c_{5}\left[\left(A_{5}-\sqrt{3}A_{8}\right)\left(p_{x}+\sqrt{3}p_{y}\right)+2A_{7}\left(p_{y}-\sqrt{3}p_{x}\right)\right]+c_{6}\left[\left(A_{1}-\sqrt{3}A_{2}\right)p_{x}+\left(\sqrt{3}A_{1}+A_{2}\right)p_{y}\right];$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{3}+c_{4}p_{z}\right)+c_{5}\left[\left(A_{5}-\sqrt{3}A_{8}\right)\left(p_{x}+\sqrt{3}p_{y}\right)+2A_{7}\left(p_{y}-\sqrt{3}p_{x}\right)\right]+c_{6}\left[A_{2}\left(p_{x}+\sqrt{3}p_{y}\right)+A_{1}\left(\sqrt{3}p_{x}-p_{y}\right)\right];$\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 230}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{c}^{v}$; $\{S_{61}^{-}|000\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}0\},\{\sigma_{z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2c}|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{6};$  & $\left(c_{1}+c_{2}k^{2}\right)\sigma_{0}+c_{3}\left[\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)+\frac{\sigma_{3}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)}{\sqrt{3}}\right];$ \tabularnewline
 & $R_{7};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{8};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{9};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
 & $R_{10};$  & $\left(c_{1}+c_{2}k^{2}\right)A_{0}+c_{3}\left[\sqrt{3}A_{5}\left(k_{x}^{2}-k_{y}^{2}\right)+A_{8}\left(k_{x}^{2}+k_{y}^{2}-2k_{z}^{2}\right)\right]+c_{4}\left(A_{4}k_{x}k_{y}+A_{6}k_{x}k_{z}+A_{7}k_{y}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{1}\left(k_{x}^{2}-k_{y}^{2}\right)\left(k_{x}^{2}-k_{z}^{2}\right)\left(k_{y}^{2}-k_{z}^{2}\right);$ \tabularnewline
 & $\{R_{8},R_{9}\};$  & $\left(c_{1}+c_{2}q^{2}\right)\Gamma_{0,0}+\left[i\alpha_{1}\Gamma_{+,0}\left(q_{x}^{2}-q_{y}^{2}+2\sqrt{2}q_{x}q_{z}\right)+2\alpha_{1}q_{y}\Gamma_{+,3}\left(q_{x}-\sqrt{2}q_{z}\right)+h.c.\right];$ \tabularnewline
 & $R_{14};$  & $c_{1}S_{0,0}+c_{2}\left(S_{2,3}k_{x}+S_{2,1}k_{y}+S_{2,2}k_{z}\right)+c_{3}\left(S_{3,7}k_{x}+S_{3,4}k_{y}-S_{3,6}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+\left[\alpha_{1}\left(q_{x}^{\prime}\Gamma_{+,0}-iq_{y}^{\prime}\Gamma_{+,3}+iq_{z}^{\prime}\Gamma_{+,1}\right)+h.c.\right];$ \tabularnewline
 & $R_{16};$  & $c_{1}\Gamma_{0,0}+(c_{2}-c_{3})\left(\Gamma_{3,2}k_{z}+\Gamma_{3,1}k_{y}\right)++\left\{ \left[2ic_{2}+(3+i)c_{3}\right]\left(k_{y}\Gamma_{+,1}-k_{z}\Gamma_{+,2}\right)+\left[(3-i)c_{2}+4ic_{3}\right]k_{x}\Gamma_{+,3}+h.c.\right\} ;$ \tabularnewline
\multirow{1}{*}{$N$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}\left(k_{x}+k_{y}\right);$ \tabularnewline

\multirow{1}{*}{$\Delta$;}&  $R_{5};$  & $\left(c_{1}+c_{2}k_{y}+c_{3}k^{2}+c_{4}k_{y}^{2}\right)\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{z}+c_{6}\sigma_{3}\left(k_{x}^{2}-k_{z}^{2}\right);$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $R_{3};$  & $\left(c_{1}+c_{2}q_{z}\right)\sigma_{0}-c_{3}(\sigma_{3}q_{x}-\sigma_{1}q_{y});$ \tabularnewline
\multirow{1}{*}{$D$;} & $R_{5};$  & $\left(c_{1}+c_{2}k_{z}\right)\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}-k_{y}\right)+c_{4}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}\right)\right]\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;}&  $R_{6};$  & $\left[c_{1}+c_{2}\left(k_{x}-k_{y}+k_{z}\right)\right]\sigma_{0}+c_{3}\sigma_{1}\left(k_{x}+k_{y}\right)-\frac{c_{3}\sigma_{3}\left(k_{x}-k_{y}-2k_{z}\right)}{\sqrt{3}};$ \tabularnewline
 &  & \tabularnewline
\multicolumn{3}{l}{Here, $\left\{ q_{x}^{\prime},q_{y}^{\prime},q_{z}^{\prime}\right\} =\left\{ \left(1+\sqrt{3}\right)k_{x}-2k_{y}+\left(\sqrt{3}-1\right)k_{z},\left(1-\sqrt{3}\right)k_{x}-2k_{y}-\left(1+\sqrt{3}\right)k_{z},-2k_{x}-2k_{y}+2k_{z}\right\} $.}\tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right)+c_{5}\sigma_{1}\left(k_{x}-k_{y}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left[c_{1}+c_{2}\left(k_{x}+k_{y}\right)\right]+c_{3}\sigma_{3}\left(k_{x}+k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{z}-A_{2}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{1}k_{x}+A_{2}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{x}+A_{1}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{y}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}k_{y}+c_{4}\left(A_{2}k_{z}-A_{1}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}q_{z}\right)+\sigma_{3}c_{3}q_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{1}q_{x}+A_{2}q_{y}\right);$\tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}q_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{3}q_{z}+c_{4}\left(A_{5}q_{x}-\sqrt{3}A_{8}q_{x}+2A_{7}q_{y}\right)+c_{5}\left(A_{2}q_{x}-A_{1}q_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}p_{z}\right)+c_{3}\sigma_{3}p_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{3}p_{z}\right)+c_{4}\left[\left(A_{5}-\sqrt{3}A_{8}\right)\left(p_{x}+\sqrt{3}p_{y}\right)+2A_{7}\left(\sqrt{3}p_{x}-p_{y}\right)\right]+c_{5}\left[\left(A_{1}+\sqrt{3}A_{2}\right)p_{x}+\left(\sqrt{3}A_{1}-A_{2}\right)p_{y}\right]$\tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}p_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)\left(c_{3}+c_{4}p_{z}\right)+c_{5}\left[\left(A_{5}-\sqrt{3}A_{8}\right)\left(p_{x}+\sqrt{3}p_{y}\right)+2A_{7}\left(\sqrt{3}p_{x}-p_{y}\right)\right]+c_{6}\left[A_{2}\left(p_{x}+\sqrt{3}p_{y}\right)+A_{1}\left(p_{y}-\sqrt{3}p_{x}\right)\right]$\tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG31.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 31}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline

\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{2}\sigma_{2}k_{y}+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 32}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}\frac{1}{2}0\},\{\sigma_{y}|0\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 33}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{\sigma_{y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $\left(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{5},R_{5}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,1}k_{x}+c_{3}\Gamma_{0,3}k_{y}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,0}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\Gamma_{3,0}k_{y}+c_{4}\Gamma_{1,0}k_{x}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{2,i}k_{x}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 34}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}\frac{1}{2}0\},\{\sigma_{y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$Q$; & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 35}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{6}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{6}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 36}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|00\frac{1}{2}\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline



\multirow{1}{*}{$A$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$H$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1},R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\Gamma_{3,0}k_{x}+c_{4}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{0,i}k_{z}+c_{i,3}\Gamma_{3,i}k_{z}\right);$\tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 37}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{\sigma_{y}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline





\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
$\Lambda$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
$H$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 38}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2y}|000\},\{\sigma_{x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
$\Delta$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$B$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$F$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 39}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2y}|000\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i}$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
$\Delta$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$B$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$G$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$F$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 40}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2y}|000\},\{\sigma_{x}|00\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline





\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
$\Delta$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
$F$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG41.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 41}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2y}|000\},\{\sigma_{x}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{3};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\left(c_{4}\sigma_{1}-c_{5}\sigma_{2}\right)k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 42}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 43}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|00\frac{1}{2}\},\{\sigma_{y}|\frac{1}{2}00\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline


\multirow{1}{*}{$C$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}+c_{5}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}+c_{5}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 44}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 45}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{y}+c_{3}k_{z})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$W$;} & $\{R_{1},R_{1}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline
 & $\{R_{2},R_{2}\};$  & $c_{1}\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline





\multirow{1}{*}{$D$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 46}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{\sigma_{y}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}k_{y}+c_{3}k_{z})\sigma_{3};$ \tabularnewline

\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}+c_{2}\sigma_{3}k_{z};$ \tabularnewline





\multirow{1}{*}{$D$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{3}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline



\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{1}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{1}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 47}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 48}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$P$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\left(c_{1}+c_{2}k_{x}\right)+\sigma_{3}\left(c_{3}+c_{4}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\left(c_{1}+c_{2}k_{x}\right)+\sigma_{3}\left(c_{3}+c_{4}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$E$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\left(c_{1}+c_{2}k_{x}\right)+\sigma_{3}\left(c_{3}+c_{4}k_{x}\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\left(c_{1}+c_{2}k_{x}\right)+\sigma_{3}\left(c_{3}+c_{4}k_{x}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 49}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 50}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG51.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 51}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline



\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline




\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 52}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+c_{3}\Gamma_{3,1}k_{y}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 53}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\{I|\frac{1}{2}00\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{y})k_{z};$ \tabularnewline


\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}-c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}-c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 54}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|000\},\{I|0\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+c_{3}\Gamma_{3,1}k_{y}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+c_{3}\Gamma_{3,1}k_{y}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{z};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $R_{5};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{3}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 55}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline


\multirow{1}{*}{$C$;} & $\{R_{2},R_{4}\};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{2}k_{x}+c_{1})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline


\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{2}k_{z}+c_{1})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y}$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{2}k_{z}+c_{1})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{1,1}+c_{5}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 56}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{x}+c_{2}\Gamma_{0,2}k_{y}+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y}+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{2}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{2}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y}$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{2}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{3},R_{4}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\left[\Gamma_{i,0}c_{i,1}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\left[\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{1,1}+c_{5}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 57}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|0\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2})k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2})k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline


\multirow{1}{*}{$C$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{2}+c_{4}\sigma_{1})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{2}+c_{4}\sigma_{1})k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{2}+c_{4}\sigma_{1})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{2}+c_{4}\sigma_{1})k_{y};$ \tabularnewline


\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{5}k_{z})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,2}k_{x}+c_{i,2}\Gamma_{i,1}k_{y});$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 58}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{y}+c_{3}\sigma_{1}k_{z})k_{x};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{y}+c_{3}\sigma_{1}k_{z})k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{x}+c_{3}\sigma_{1}k_{z})k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y}$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y}$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{1,1}+c_{5}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 59}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline

\multirow{1}{*}{$U$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{3}\sigma_{3}k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline


\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline


\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y}$ \tabularnewline
 & $\{R_{3},R_{4}\};$  & $(c_{1}+c_{2}k_{z}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{y}$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1},R_{2}\right\} ,\left\{ R_{3},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right)+k_{y}\left(c_{4}\Gamma_{1,1}+c_{5}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 60}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|000\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}0\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{y}+c_{3}\sigma_{1}k_{z})k_{x};$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{3}k_{y}+c_{3}\sigma_{1}k_{z})k_{x};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y}+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{x}+c_{2}\Gamma_{0,2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+\sum_{i=1}^{2}c_{i,1}\Gamma_{i,2}k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{1},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{5}k_{z})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,1}k_{x}+c_{i,2}\Gamma_{i,2}k_{y});$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{5}\right\} ,\left\{ R_{5}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{x}+\Gamma_{1,0}\left(c_{2}+c_{3}k_{x}\right)+\left(c_{4}\Gamma_{0,3}+c_{5}\Gamma_{1,3}+c_{6}\Gamma_{3,3}\right)k_{y}+c_{7}\Gamma_{2,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{8}\right\} ,\left\{ R_{4},R_{6}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\left[\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,0}+c_{3}\Gamma_{2,3}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{1},R_{4}\right\} ,\left\{ R_{2},R_{3}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG61.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 61}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{0,2}k_{x}+(c_{3}\Gamma_{1,2}+c_{4}\Gamma_{2,2})k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+(c_{2}\Gamma_{1,2}+c_{3}\Gamma_{2,2})k_{y}+c_{4}\Gamma_{0,2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+(c_{2}\Gamma_{1,2}+c_{3}\Gamma_{2,2})k_{x}+c_{4}\Gamma_{0,2}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\Gamma_{0,0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,3}k_{x}k_{y}+\sum_{i=1}^{3}(c_{i,2}\Gamma_{i,1}k_{x}k_{z}+c_{i,3}\Gamma_{i,2}k_{y}k_{z});$ \tabularnewline
 & $\{R_{10},R_{10}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\Gamma_{0,0}+\sum_{i=1}^{3}c_{i,1}\Gamma_{i,3}k_{x}k_{y}+\sum_{i=1}^{3}(c_{i,2}\Gamma_{i,1}k_{x}k_{z}+c_{i,3}\Gamma_{i,2}k_{y}k_{z});$ \tabularnewline

\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{2}k_{y})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,3}k_{x}+c_{i,2}\Gamma_{i,1}k_{z});$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{2}k_{x})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,1}k_{y}+c_{i,2}\Gamma_{i,3}k_{z});$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{2}k_{z})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,1}k_{x}+c_{i,2}\Gamma_{i,3}k_{y});$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{2}\sigma_{1}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & \multicolumn{1}{l}{$\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$ } & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$H$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 62}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z}$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z}$ \tabularnewline
 & $\{R_{10},R_{12}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z}$ \tabularnewline
 & $\{R_{14},R_{16}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{z}$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{2}\sigma_{3}k_{y}k_{z}$ \tabularnewline
 & $R_{10};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+c_{2}\sigma_{3}k_{y}k_{z}$ \tabularnewline
\multirow{1}{*}{$S$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{3}\Gamma_{3,1}k_{x}+(c_{4}\Gamma_{1,2}+c_{2}\Gamma_{2,2})k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{9},R_{10}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\Gamma_{3,1}k_{x}+c_{3}\Gamma_{0,2}k_{y};$ \tabularnewline

\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{z};$ \tabularnewline
 & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$C$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$E$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}k_{z};$ \tabularnewline
 & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\{R_{5},R_{5}\};$  & $(c_{1}+c_{2}k_{z})\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,3}k_{x}+c_{i,2}\Gamma_{i,1}k_{y});$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{1},R_{3}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}c_{i,1}\Gamma_{i,0}k_{y}+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{z}\left(c_{4}\Gamma_{1,0}+c_{5}\Gamma_{2,3}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$C$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{y}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{z}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$E$;} & $\left\{ R_{2},R_{6}\right\} ,\left\{ R_{4},R_{8}\right\} ;$  & $c_{1}\Gamma_{0,0}+\sum_{i=0,3}\Gamma_{i,0}c_{i,1}k_{x}+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right)+k_{z}\left(c_{4}\Gamma_{1,0}+c_{5}\Gamma_{2,3}\right);$ \tabularnewline
\multirow{1}{*}{$A$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{x}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{z}+k_{x}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{y}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 63}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|00\frac{1}{2}\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline

\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline



\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 64}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|00\frac{1}{2}\},\{C_{2y}|00\frac{1}{2}\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{x}k_{y}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+\sum_{i=1}^{2}\sigma_{i}(c_{i,1}k_{x}+c_{i,2}k_{y})k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{4}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{4}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$B$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multirow{1}{*}{$G$;} & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{6},R_{8}\right\} ;$  & $c_1\Gamma_{0,0}+\sum_{i=0,3}\left[c_{i,1}\Gamma_{i,0}k_{y}+k_{z}\left(c_{i,2}\Gamma_{i,1}+c_{i,3}\Gamma_{i,2}\right)\right]+k_{x}\left(c_{2}\Gamma_{1,1}+c_{3}\Gamma_{1,2}\right);$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 65}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 66}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline





\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{4}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2}+c_{4}\sigma_{3}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 67}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline








\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$E$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 68}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{b}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{4}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{3}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{4}\sigma_{2}k_{x}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\multirow{1}{*}{$E$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{4}\sigma_{2}k_{y}+c_{3}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 69}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$H$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$C$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$A$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}[t]
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$B$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 70}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{f}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{4}\frac{1}{4}\frac{1}{4}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline

\multirow{1}{*}{$Y$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$G$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$H$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline


\multirow{1}{*}{$C$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{1}k_{y}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+c_{3}\sigma_{2}k_{y}+c_{4}\sigma_{1}k_{z};$ \tabularnewline


\multirow{1}{*}{$D$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{1}k_{x}+c_{4}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$B$;} & $R_{5};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$R$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG71.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 71}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline















\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sigma_{1}\left(c_{5}k_{y}+c_{6}k_{z}\right);$ \tabularnewline
$\Delta$; & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sigma_{1}\left(c_{5}k_{x}+c_{6}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 72}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|000\},\{C_{2y}|000\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{y}+c_{3}k_{z})\sigma_{2};$ \tabularnewline

\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{z};$ \tabularnewline
 & $\{R_{3},R_{4}\};$  & $c_{1}\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{z};$ \tabularnewline





\multirow{1}{*}{$D$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 73}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|000\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline


\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{z})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$S$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{y}+c_{3}k_{z})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{9},R_{9}\};$  & $2c_{1}\Gamma_{0,0}+\sum_{i=1}^{3}(c_{i,1}\Gamma_{i,2}k_{x}+c_{i,2}\Gamma_{i,3}k_{y}+c_{i,3}\Gamma_{i,1}k_{z});$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$D$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{y}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Q$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{z})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 74}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{o}^{v}$; $\{C_{2z}|\frac{1}{2}0\frac{1}{2}\},\{C_{2y}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline




\multirow{1}{*}{$T$;} & $R_{5};$  & $c_{1}\sigma_{0}+(c_{2}k_{x}+c_{3}k_{y})\sigma_{2};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{9};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{x}+c_{3}\sigma_{3}k_{y};$ \tabularnewline


\multirow{1}{*}{$P$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$G$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multicolumn{1}{l}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{4}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{1}k_{y};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x};$ \tabularnewline
\multirow{1}{*}{$D$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+\sigma_{1}\left(c_{5}k_{y}+c_{6}k_{z}\right);$ \tabularnewline
\multicolumn{1}{l}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multicolumn{1}{l}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sigma_{1}\left(c_{5}k_{x}+c_{6}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 75}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline











\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{}\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 76}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{4}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 77}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline











\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 78}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{3}{4}\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $\{R_{2},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{2},R_{8}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
 & $\{R_{4},R_{6}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{1}\};$  & $(c_{1}+c_{2}k_{x}+c_{3}k_{y})\sigma_{0}+\sum_{i=1}^{3}c_{i,1}\sigma_{i}k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 79}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})+c_{i,3}k_{z}\right]\sigma_{i};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 80}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{2}\};$  & $c_{1}\sigma_{0}+c_{3}(\sigma_{2}k_{x}+\sigma_{1}k_{y})+c_{4}(\sigma_{1}k_{x}-\sigma_{2}k_{y})+c_{2}\sigma_{3}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{+}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(\alpha_{1}\sigma_{+}k_{-}+h.c.\right);$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG81.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 81}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{S_{4z}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left(A_{4}c_{3}+A_{6}c_{4}-A_{1}c_{6}-A_{2}c_{7}\right)k_{x}+\left(-A_{6}c_{3}+A_{4}c_{4}-A_{2}c_{6}+A_{1}c_{7}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left(A_{4}c_{3}+A_{6}c_{4}-A_{1}c_{6}-A_{2}c_{7}\right)k_{x}+\left(-A_{6}c_{3}+A_{4}c_{4}-A_{2}c_{6}+A_{1}c_{7}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 82}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{S_{4z}^{+}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
 & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k^{2}+c_{3}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{2}\};$  & $(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2})\sigma_{0}+\sum_{i=1}^{3}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left(A_{4}c_{3}+A_{6}c_{4}-A_{1}c_{6}-A_{2}c_{7}\right)k_{x}+\left(-A_{6}c_{3}+A_{4}c_{4}-A_{2}c_{6}+A_{1}c_{7}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{2}\right\} ;$  & $A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z}+\left(A_{4}c_{3}+A_{6}c_{4}-A_{1}c_{6}-A_{2}c_{7}\right)k_{x}+\left(-A_{6}c_{3}+A_{4}c_{4}-A_{2}c_{6}+A_{1}c_{7}\right)k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 83}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{I|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 84}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{I|00\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 85}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}0\},\{I|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{7}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline




\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{2}-A_{3}\right)c_{4}\right]k_{x}+\left[\left(A_{3}-A_{2}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 86}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\{I|\frac{1}{2}\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$M$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{7}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline




\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}+c_{i,2}k_{y})\sigma_{i};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{2}-A_{3}\right)c_{4}\right]k_{x}+\left[\left(A_{3}-A_{2}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}\left(c_{5}+c_{6}k_{z}\right);$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 87}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{I|000\},\mathcal{T}$; Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})+c_{i,3}k_{z}\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline







\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\sigma_{1}\left(c_{4}k_{x}+c_{5}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 88}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\{I|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\mathcal{T}$;
Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline

\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+\sigma_{2}\left(c_{2}k_{x}+c_{3}k_{y}\right);$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3};$ \tabularnewline
 & $R_{10};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\left[c_{4}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $\{R_{1},R_{4}\};$  & $c_{2}(\sigma_{2}k_{x}+\sigma_{1}k_{y})+c_{3}(\sigma_{1}k_{x}+\sigma_{2}k_{y})+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{2},R_{3}\};$  & $c_{2}(\sigma_{2}k_{x}+\sigma_{1}k_{y})+c_{3}(\sigma_{1}k_{x}+\sigma_{2}k_{y})+c_{1}\sigma_{0};$ \tabularnewline
\multirow{1}{*}{$\Lambda$;}&  $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$V$;} & $\{R_{5},R_{7}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}\left[c_{i,1}k_{x}k_{y}+c_{i,2}(k_{x}^{2}-k_{y}^{2})\right]\sigma_{i};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{4}k_{x}+c_{3}k_{y})\sigma_{1}+(c_{6}k_{x}+c_{5}k_{y})\sigma_{2};$ \tabularnewline






\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{2},R_{4}\right\} ,\left\{ R_{3}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5},R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\left[\left(A_{4}+A_{6}\right)c_{3}+\left(A_{2}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{1}-A_{2}\right)c_{3}+\left(A_{4}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\left[\left(A_{6}+A_{7}\right)c_{3}+\left(A_{3}-A_{2}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{3}\right)c_{3}+\left(A_{6}+A_{7}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+A_{8}c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{3}k_{y}\right)+\sigma_{3}\left(c_{4}k_{x}+c_{5}k_{y}\right)+c_{6}\sigma_{1}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 89}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\mathcal{T}$; Non-Centrosymmetric;
without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline











\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 90}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline



\multirow{1}{*}{$V$;} & $\{R_{1},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{llp{15cm}<{\raggedright}l}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+\left\{ (1+i)\left[\left(c_{4}\Gamma_{+,0}+ic_{5}\Gamma_{+,3}\right)k_{-}+ik_{+}\left(c_{6}\Gamma_{+,1}+c_{7}\Gamma_{+,2}\right)\right]+h.c.\right\} ;$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}

==> dSG/basicinfo/merge/mergeSG91.tex <==
{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 91}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{4}\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 92}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{4}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{6},R_{7}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[\Gamma_{0,2}(k_{x}-k_{y})+\Gamma_{3,3}(k_{x}+k_{y})\right]+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{2},R_{6}\};$  & $(c_{1}+c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+\left\{ (1+i)\left[\left(c_{4}\Gamma_{+,0}+ic_{5}\Gamma_{+,3}\right)k_{-}+ik_{+}\left(c_{6}\Gamma_{+,1}+c_{7}\Gamma_{+,2}\right)\right]+h.c.\right\} ;$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+\Gamma_{3,0}c_{3}k_{x}+c_{4}\Gamma_{1,0}k_{z}+c_{5}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{2,i}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 93}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline











\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 94}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{1}{2}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline



\multirow{1}{*}{$V$;} & $\{R_{1},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{5}\sigma_{1}+c_{6}\sigma_{2})k_{x}k_{y};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+\left\{ (1+i)\left[\left(c_{4}\Gamma_{+,0}+ic_{5}\Gamma_{+,3}\right)k_{-}+ik_{+}\left(c_{6}\Gamma_{+,1}+c_{7}\Gamma_{+,2}\right)\right]+h.c.\right\} ;$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 95}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{3}{4}\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline



\multirow{1}{*}{$S$;} & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$T$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 96}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|00\frac{3}{4}\},\{C_{2x}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+(c_{4}\sigma_{1}+c_{5}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{3}k_{x}k_{y};$ \tabularnewline
\multirow{1}{*}{$Z$;} & $R_{6};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
 & $R_{7};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{6},R_{7}\};$  & $c_{1}\Gamma_{0,0}+c_{2}\left[\Gamma_{0,2}(k_{x}-k_{y})+\Gamma_{3,3}(k_{x}+k_{y})\right]+c_{3}\Gamma_{3,1}k_{z};$ \tabularnewline
\multirow{1}{*}{$R$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
 & $\{R_{6},R_{8}\};$  & $(c_{1}+\sum_{i=x}^{z}c_{i}k_{i}^{2})\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline

\multirow{1}{*}{$U$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline

\multirow{1}{*}{$V$;} & $\{R_{1},R_{3}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline
 & $\{R_{2},R_{4}\};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+(c_{2}\sigma_{1}+c_{3}\sigma_{2})k_{x}k_{y};$ \tabularnewline

\multirow{1}{*}{$S$;} & $\{R_{4},R_{8}\};$  & $(c_{1}+c_{2}k_{x}+c_{2}k_{y})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{z};$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{2}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
 & $\{R_{4},R_{4}\};$  & $\left(c_{1}+c_{2}k_{x}+\sum_{i=x}^{z}c_{i}k_{i}^{2}\right)\sigma_{0}+\sum_{i=1}^{3}c_{i}\sigma_{i}k_{y}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $\{R_{1},R_{2}\};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+(c_{3}\sigma_{1}+c_{4}\sigma_{2})k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$V$;} & $\left\{ R_{1},R_{3}\right\} ,\left\{ R_{2},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\Gamma_{3,0}k_{z}+\left\{ (1+i)\left[\left(c_{4}\Gamma_{+,0}+ic_{5}\Gamma_{+,3}\right)k_{-}+ik_{+}\left(c_{6}\Gamma_{+,1}+c_{7}\Gamma_{+,2}\right)\right]+h.c.\right\} ;$\tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{2},R_{2}\right\} ,\left\{ R_{4},R_{4}\right\} ;$  & $\Gamma_{0,0}\left(c_{1}+c_{2}k_{x}\right)+\Gamma_{3,0}c_{3}k_{x}+c_{4}\Gamma_{1,0}k_{z}+c_{5}\Gamma_{2,0}k_{y}+\sum_{i=1}^{3}\left(c_{i,1}\Gamma_{1,i}k_{y}+c_{i,2}\Gamma_{2,i}k_{z}\right);$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 97}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|000\},\{C_{2x}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;}&  $\{R_{3},R_{4}\};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+\sum_{i=1}^{2}(c_{i,1}k_{x}k_{y}+c_{i,2}k_{z})\sigma_{i}+c_{4}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 98}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}^{v}$; $\{C_{4z}^{+}|\frac{3}{4}\frac{1}{4}\frac{1}{2}\},\{C_{2x}|0\frac{1}{2}\frac{1}{2}\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline


\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3}+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\multirow{1}{*}{$P$;} & $R_{10};$  & $c_{1}\sigma_{0}+c_{2}(\sigma_{2}k_{x}-\sigma_{3}k_{y})+c_{3}\sigma_{1}k_{z};$ \tabularnewline









\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1-i)c_{5}\sigma_{+}k_{+}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}+c_{3}k^{2}+c_{4}k_{z}^{2}\right)+\sigma_{3}\left(c_{5}k_{z}+c_{6}k^{2}+c_{7}k_{z}^{2}\right)+\left[\sigma_{+}\left(\alpha_{1}k_{+}^{2}+\alpha_{2}k_{-}^{2}\right)+h.c.\right];$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left[(1+i)c_{5}\sigma_{+}k_{-}+h.c.\right];$ \tabularnewline
\multirow{1}{*}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+c_{5}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$F$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{6}\sigma_{2}k_{y}+c_{5}\sigma_{1}k_{z};$ \tabularnewline
\multirow{1}{*}{$Q$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+\sum_{i=1}^{2}\sigma_{i}\left(c_{i,1}k_{x}+c_{i,2}k_{z}\right);$ \tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{1}k_{z}+c_{5}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}-c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}-c_{3}k_{y}\right)+c_{4}\sigma_{1}\left(k_{x}+k_{y}\right)+c_{6}\sigma_{2}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 99}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|000\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline




\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline





\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$\tabularnewline
\multirow{1}{*}{$Y$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}\right)+c_{3}\sigma_{3}k_{x}+c_{5}\sigma_{2}k_{y};$\tabularnewline
\multicolumn{1}{l}{$W$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{y};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z}+\left(c_{5}\sigma_{1}+c_{6}\sigma_{2}\right)k_{x};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%
\begin{table*}
\raggedright{}%
\begin{tabular}{lll}
\multicolumn{3}{l}{SG 100}\tabularnewline
\hline
\multicolumn{3}{l}{$\Gamma_{q}$; $\{C_{4z}^{+}|000\},\{\sigma_{y}|\frac{1}{2}\frac{1}{2}0\},\mathcal{T}$;
Non-Centrosymmetric; without SOC }\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Gamma$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{1}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$M$;} & $\{R_{5},R_{6}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$Z$;}&  $R_{5};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}\sigma_{1}k_{x}k_{y}+c_{5}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$A$;} & $\{R_{5},R_{6}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $\{R_{7},R_{8}\};$  & $c_{2}\sigma_{3}k_{z}+c_{1}\sigma_{0};$ \tabularnewline
 & $R_{9};$  & $\left[c_{1}+c_{2}(k_{x}^{2}+k_{y}^{2})+c_{3}k_{z}^{2}\right]\sigma_{0}+c_{4}k_{x}k_{y}\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$R$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline
\multirow{1}{*}{$X$;} & $R_{5};$  & $c_{1}\sigma_{0}+c_{2}\sigma_{2}k_{y};$ \tabularnewline


\multirow{1}{*}{$\Lambda$;}&  $R_{5};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{1}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{3};$ \tabularnewline
\multirow{1}{*}{$V$;}&  $R_{9};$  & $\left[c_{1}+c_{2}k_{z}+c_{3}(k_{x}^{2}+k_{y}^{2})+c_{4}k_{z}^{2}\right]\sigma_{0}+c_{5}\sigma_{3}k_{x}k_{y}+c_{6}(k_{x}^{2}-k_{y}^{2})\sigma_{2};$ \tabularnewline


\multirow{1}{*}{$Y$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{5}\sigma_{2})k_{y}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$T$;} & $\{R_{2},R_{4}\};$  & $(c_{1}+c_{2}k_{x})\sigma_{0}+(c_{3}\sigma_{1}+c_{5}\sigma_{2})k_{y}+c_{4}\sigma_{3}k_{z};$ \tabularnewline
\multirow{1}{*}{$W$;} & $R_{5};$  & $(c_{1}+c_{2}k_{z})\sigma_{0}+c_{3}\sigma_{2}k_{x}+c_{4}\sigma_{1}k_{y};$ \tabularnewline
\end{tabular}
\end{table*}

}{
\global\long\def\arraystretch{1.4}%

\begin{table*}
\raggedright{}%
\begin{tabular}{lll}

\hline
\multicolumn{3}{l}{Symmetry-protected accidental points at high symmetry line}\tabularnewline
\multicolumn{3}{l}{ }\tabularnewline
\multirow{1}{*}{$\Delta$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$ \tabularnewline
\multirow{1}{*}{$U$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{y}\right)+c_{3}\sigma_{3}k_{y}+c_{5}\sigma_{1}k_{x};$\tabularnewline
\multicolumn{1}{l}{$\Lambda$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{1}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{4}c_{3}-A_{1}c_{5}\right)k_{x}+\left(A_{2}c_{5}-A_{6}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{3}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{2}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{2}k_{x}+A_{1}k_{y}\right)+c_{3}\left(A_{6}k_{x}+A_{4}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{4}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{3}\right\} ,\left\{ R_{5}\right\} ;$  & $c_{5}\left(A_{1}k_{x}+A_{2}k_{y}\right)+c_{3}\left(A_{4}k_{x}+A_{6}k_{y}\right)+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
 & $\left\{ R_{4}\right\} ,\left\{ R_{5}\right\} ;$  & $\left(A_{6}c_{3}-A_{2}c_{5}\right)k_{x}+\left(A_{1}c_{5}-A_{4}c_{3}\right)k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{4}k_{z};$ \tabularnewline
\multicolumn{1}{l}{$V$;} & $\left\{ R_{5}\right\} ,\left\{ R_{6}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{5}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{7}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{6}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{8}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{z}\right)+c_{3}\sigma_{3}k_{z};$ \tabularnewline
 & $\left\{ R_{7}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{6}-A_{1}\right)c_{4}\right]k_{x}+\left[\left(A_{2}-A_{4}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
 & $\left\{ R_{8}\right\} ,\left\{ R_{9}\right\} ;$  & $\left[\left(A_{4}-A_{2}\right)c_{3}+\left(A_{1}+A_{6}\right)c_{4}\right]k_{x}+\left[\left(A_{2}+A_{4}\right)c_{3}+\left(A_{1}-A_{6}\right)c_{4}\right]k_{y}+A_{0}\left(c_{1}+c_{2}k_{z}\right)+\left(\sqrt{3}A_{5}+A_{8}\right)c_{5}k_{z};$ \tabularnewline
\multirow{1}{*}{$\Sigma$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$ \tabularnewline
\multirow{1}{*}{$S$;} & $\left\{ R_{1}\right\} ,\left\{ R_{2}\right\} ;$  & $\sigma_{0}\left(c_{1}+c_{2}k_{x}+c_{2}k_{y}\right)+\sigma_{3}\left(c_{3}k_{x}+c_{3}k_{y}\right)+c_{4}\sigma_{2}\left(k_{y}-k_{x}\right);$\tabularnewline
\end{tabular}
\end{table*}

}
